Tightly Seal Your Sensitive Pointers with PACTight

ARM is becoming more popular in desktops and data centers, opening a new realm in terms of security attacks against ARM. ARM has released Pointer Authentication, a new hardware security feature that is intended to ensure pointer integrity with cryptographic primitives. In this paper, we utilize Pointer Authentication (PA) to build a novel scheme to completely prevent any misuse of security-sensitive pointers. We propose PACTight to tightly seal these pointers. PACTight utilizes a strong and unique modifier that addresses the current issues with the state-of-the-art PA defense mechanisms. We implement four defenses based on the PACTight mechanism. Our security and performance evaluation results show that PACTight defenses are more efficient and secure. Using real PA instructions, we evaluated PACTight on 30 different applications, including NGINX web server, with an average performance overhead of 4.07% even when enforcing our strongest defense. PACTight demonstrates its effectiveness and efficiency with real PA instructions on real hardware.

==> README <==
die: a paper template
=====================

## start

0. Prerequisites

  - Python 3.x
  - pygmentize

    $ pip install Pygments 

1. clone the git repo:

  - if you have none,

    $ git clone --depth=1 git@github.com:tsgates/die.git

  - if you have a git-repo to work on,

    $ git subtree add --squash git@github.com:tsgates/die.git master -P paper

  - or

    $ wget https://github.com/tsgates/die/releases/download/latest/die.tar.gz

2. build it:

    $ make
    p.pdf built @Tue May 20 20:38:19 EDT 2014
    
    (check p.pdf)

3. starting point, p.tex:

    $ grep -oP 'input{\K\w+' p.tex
    cmds
    rev
   *hdr
    abstract
   *ex
    intro
    overview
    design
    impl
    eval
    conclusion
    ack

  - hdr: includes title/author info
  - ex : includes latex examples

4. example latex

    $ git checkout example
    $ make

5. formatting rules (dependencies)

  - code/*.{c,cc,py,js ...} -> code/*.tex
  - fig/*.svg               -> fig/*.pdf
  - data/*.gp               -> fig/*.tex

  (see ex.tex for more details)

## tools

1. make a draft for revision

    $ make draft
    $ make watermark

2. abstract.txt (from abstract.tex)

    $ cat abstract.txt 

3. highlight changes, since the last submit

    $ make diff DIFF=HEAD@{}

4. spell check

    $ make spell

## Acknowledgment

This template contains a few files copied/stolen from the Internet and
mainly from my past collaborators (e.g., sty/*, conf.bib, some bin/),
which I couldn't keep track of their licenses.

==> _bg.tex <==
\section{Background and Motivation}
\label{s:bg}

\CM{Since this is a big section, you need a short intro to the section
explaining what are subections and why you want to have such subsections as
a guide to read this long section.}

%%%%
\subsection{Memory Corruption}
\label{s:bg:memory}

\CM{I think we'd remove this section because it can give wrong impression that
we aim to defend all memory corruption attacks. I suggest to merge this section
to \autoref{s:bg:control} and focus on the memory corruption attacks causing
control flow hijacking.
}
Memory corruption vulnerabilities have long been one 
of the main avenues attackers choose to attack systems.
The basis of most systems is written in unsafe C and 
C++ languages that are prone to many memory corruption 
vulnerabilities, due to the inexistence of sanity checks. 
Thus, an attacker may exploit the language semantics
to corrupt the memory, and even craft their own attacks 
with calculated corruptions. The first buffer overflow attack
was documented in 1972, and since then, there has been 
many attacks and defenses by both red and blue teams. More than 30
years later, and the problem is still prevalent. According 
to Microsoft, in 2018, more than 70\% of its CVEs 
were memory-corruption related, with many of these being 
critical. Attackers have become very innovative in their attacks,
with attacks such as ROP, heap spraying and COOP attacks. 

%%%%
\subsection{Control Flow Attacks}
\label{s:bg:control}

A control-flow hijacking attack is carried out by attackers 
by exploiting a memory corruption error to overwrite a code 
pointer (return addresses and function pointers) to subvert 
the flow of the program. Due to the existence of DEP, code injection 
attacks are no longer possible. However, attackers can achieve 
arbitrary code execution by carefully stitching these subversions. 
Corrupting the return address can be used to achieve ROP attacks. 
ROP attacks that are performed without corrupting return addresses
are referred to as JOP. In C++, corrupting VTable pointers can 
achieve type confusion attacks on C++, such as VTable hijacking 
and COOP. Thus, our goal is to provide a protection scheme able 
to protect against all these attacks, in addition to provide protection
to the data pointers pointing to all the code pointers. Our goal 
is to tightly seal these pointers to provide a robust protection against
all these different classes of attacks.

\MI{Needs to be rewritten}
A popular class of memory attacks referred to as control-flow 
hijacking attacks. These are attacks in which the attacker 
subverts the program's control flow to a malicious one to achieve 
certain goals such as arbitrary code execution (ACE). 
This can be done by exploiting memory corruption errors such as 
buffer overflows, use-after-free and format string vulnerabilities.
In order to combat these attacks, there have been many solutions 
and techniques proposed. One of the most prominent 
is CFI. CFI protects mainly against control-flow hijacking 
attacks. The main premise is that a program must conform to a 
CFG. If the program conforms to that CFG, then it's valid and 
protected. This is mainly done by protecting indirect code 
pointers (Forward edge) and return addresses (backward edge). 
There have been many CFI mechanisms propoosed. However, there
is always a caveat. CFI mechanisms are usually either efficient 
but imprecise (coarse grained) or inefficient but precise 
(fine grained). Many methods make the best effort to strike 
the balance between them. Although there is only one legitimate 
target that should be allowed at each call/jump site at a 
specific runtime, these methods inherently have a large equivalence 
class (EC) size (i.e., number of allowed legitimate targets 
at one call site). A state-of-the-art implementation of CFI, 
OS-CFI, has an indirect call site that allows 427 legitimate 
call targets in SPEC CPU2006.

On ARM, there is a dedicated Link Register (LR) that stores the return 
address. Even though the attacker cannot directly manipulate
the contents of the LR, however the existence of nested function calls 
on the stack requires the LR to be stored on the stack, so that 
the next function call can replace the value of the LR with its 
return address. It is during this window that the attacker can corrupt the
return address and subvert the control-flow.

\CM{
This paragraph is the perfect place to briefly introduce the defenses that we
implemented. It will be good to introduce CFI, CFIXX-like vtable protection,
CPI, and return address protection as representative defense mechanisms against
control flow attacks.
}
CFI is one of the most popular defenses against control flow attacks. 
The goal of CFI is for the program to conform to a specific 
CFG, that is statically or dynamically generated. This guarantees 
the integrity of the program flow. Current CFI techniques suffer are 
either imprecise and efficient (coarse-grained) or precise and 
inefficient (fine-grained).
  

%%%%
\subsection{ARM Pointer Authentication}
\label{s:bg:arm}

\MI{Tables and figures - Figure 1: PAC mechanism for signing. Figure 2: PAC mechanism for authenticating.
Table 1: PAC instructions with small explanantion (similar to PTAuth)}

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figs/pac-sign}
	\caption{
		PAC signing mechanism.
        \CM{
        - Please do not use textbf in the caption.
        - By default, use Times New Roman font inside fig. You can install
        a times new roman to your linux laptop. See
        \url{https://www.fosslinux.com/42406/how-to-install-microsoft-truetype-fonts-on-fedora.htm}
        }
	}
%	\vspace{-1.5em}
	\label{f:sign}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figs/pac-auth}
	\caption{
		\textbf{PAC authenticating mechanism}
	}
%	\vspace{-1.5em}
	\label{f:auth}
\end{figure}


\begin{table}[t]
  \centering
  \resizebox{\columnwidth}{!}{\input{figs/tbl-pac-instr.tex}}

  \caption{PAC instructions
    %
    \CM{Formatting all the tables this way: 1) create a separate tex file for
    each table (it is less distracted in reading the tex) , 2) include it
    inside the resizebox, 3) use "t:" fore label prefix, and 4) use cc tag for
    all machine instructions in the paper.}
    %
  }

  \label{t:pac-instr}
\end{table}

\CM{Fig 2 is not referenced? All figures and tables must be referenced in the
text.}

\CM{This section is hard to follow. One reason is that you referenced Table
1 in the text but the table does not provide much information. For example,
  what is A/B.Code/Data?}

ARMv8.3 introduced a new and promising hardware security feature 
called Pointer Authentication (PA). PA is implemented in
AArch64, ARM's 64-bit state. PA instructions are considered as NOP 
instructions in older architectures, thus providing backwards compatibility. 
PA's main aim is to provide integrity to pointers, and be able to detect 
malicious overwrites of pointers.

PA defines hardware instructions for generating and authenticating 
Pointer Authentication Codes (PACs). These PACs, similar to 
Message Authentication Codes (MACs), are cryptographically generated. 
PA utilizes the QARMA algorithm as its cryptography primitive. 
QARMA takes two 64-bit values (the pointer and modifier), as well as a 
128-bit key, and generates a 64-bit PAC. The modifier can be chosen
by the programmer and passed to the instruction, as shown by~\autoref{t:pac-instr}. 
These PACs are truncated and added to the upper unused bits of the 64-bit 
pointer, as shown by~\autoref{f:sign}. A total of five keys can be chosen 
to generate the PACs, two keys for code pointers, two keys for data pointers, 
and one generic key. These are secured and protected by the kernel. 

When authenticating, the authentication instructions (\autoref{t:pac-instr}) take the 
pointer with the PAC and the modifier. Both values need to be the same 
as the ones originally used to generate the PAC. The PAC is then 
regenerated and compared with the one on the passed pointer. If it is the 
same, the PAC is removed from the pointer and the pointer can be
used. Otherwise, the top two bits of the pointer are flipped, rendering 
the pointer unusable. Any use of the pointer in the pointer results
in a segfault. PAC has been implemented in the Apple A12 chip initially, 
and the subsequent ones, as well as recently in the newly announced
Apple M1 chip. Very recently, ARM announced ARMv8.6 with Enhanced PAC. 
This iteration of PAC features several improvements. Instead of 
flipping the top two bits of the pointer upon authentication failure, 
an exception is thrown, immediately terminating the program. In 
addition to that is that the PAC is XORed with the top bits of the 
pointer rather than just placed, which could help in mitigating some
PAC reuse attacks. At the moment, there is no publicly available 
hardware with ARMv8.6 support.


\subsection{Attacks on Pointer Authentication}
\label{s:bg:attacks}

\begin{table}[]
	\begin{tabular}{|l|c|c|c|}
		\hline
		\textbf{Defense} & \multicolumn{1}{l|}{\textbf{Property 1}} & \multicolumn{1}{l|}{\textbf{Property 2}} & \multicolumn{1}{l|}{\textbf{Property 3}} \\ \hline
		GCC              & \textbf{X}                               & \textbf{}                                & \textbf{}                                \\ \hline
		Apple Clang      & \textbf{X}                               & \textbf{}                                & \textbf{}                                \\ \hline
		PARTS            & \textbf{X}                               & \textbf{}                                & \textbf{}                                \\ \hline
		PACStack         & \textbf{X}                               & \textbf{X}                               & \textbf{}                                \\ \hline
		PCan             & \textbf{X}                               & \textbf{}                                & \textbf{}                                \\ \hline
		PTAuth           & \textbf{X}                               & \textbf{}                                & \textbf{}                                \\ \hline
		\sys             & \textbf{X}                               & \textbf{X}                               & \textbf{X}                               \\ \hline
	\end{tabular}
	\caption{Defense mechanisms and the three properties}
	\label{tab:pac-defenses}
\end{table}
%
\MI{Table 2 - All three properties and related work and how each violate it.}
%
There are several inherent weaknesses, such as using a signing gadget 
to forge PACs (Google attack), and reusing of PACs that have
the same modifier (PARTS attack). The second attack is possible with 
the default implmementation of PAC that protects the stack.

The default implementation uses PACIASP and AUTIASP. These have the 
stack pointer (SP) as the modifier. If it coincides that two
stack frames have the same stack pointer value, then PACs can be 
reused to redirect control flow. In very large programs, this 
can be achieved in a similar manner to how ROP is able to reuse 
gadgets. Thus, PAC is able to provide unforgeable pointers (Property 1),
however the pointer is still copyable (Property 2) if the modifier 
is weak. In addition to that, if a memory object is freed, but there is
still PACed pointer that points to it, this can be maliciously used 
by the attacker as well. The pointer is now dangling (Property 3) and 
a UAF attack with PAC is possible. \CM{
We did not introduce Property 1, 2, 3 yet so it is not appropriate to mention
them in this section. The goal in the background section is to reveal three
weaknesses and explain their security implications. These properties should be
presented in section 4.
}

\CM{
This paragraph should explain how state of the art PAC approaches still fail to
achieve these three properties. The important point here is linking their
weaknesses to one of three properties.
}
Previous PAC approaches focused on CFI (PARTS), DFI (PARTS), 
protecting the stack (PACStack, PCan) or achieving temporal 
safety (PTAuth). Whilst these approaches demonstrated the potential 
and effectiveness of PAC, many still weren't efficient enough 
and some had their own security concerns. PARTS-CFI was very efficient 
but only protected code pointers and had a static modifier. The modifier
was more unique than the default PAC implementation, but could still 
provide avenues for exploitation. PARTS-DFI protected all data pointers 
but was very inefficient. PARTS-DFI incurred an average overhead of 20\% 
on nbench. PACStack only protected the stack and needs a control-flow
integrity scheme with it to guarantee it's protection. PTAuth only 
achieves temporal safety and incurs an average overhead of 21\%. With the
exception of PTAuth, none of these schemes provide any notion of memory safety.

\CM{
The description on our goals should be moved to the next section.
}
Thus, our main goal is to guarantee all 3 properties (unforgeability, 
uncopyability, and non-dangling) to tightly seal PACed pointers.
Guaranteeing all 3 properties prevents all current known attacks and 
weaknesses on ARM's Pointer Authentication from happening.
Current implementations fall short on these. GCC's implementation 
uses the stack pointer (SP) as a modifier. This fails to achieve property 2.
Using the SP only as a modifier has been shown to be vulnerable to PAC 
reuse attacks. Apple's implementation implements several protections on 
a variety of pointers. However, it still uses the SP for return addresses, 
and uses 0 as a modifier for function pointers and V-Table pointers.
Thus, this also violates property 2, as an attacker can reuse these PACs 
due to the weak nature of the modifier. PARTS uses a type-id based on 
the LLVM ElementType. In spite of the fact that this does increase the 
difficulty of the attack, property 2 can still be violated. Although it
would be more difficult to exploit, two pointers can have the same LLVM 
ElementType and be exploited by an attacker. In addition to this, the
static nature of the modifier means that property 3 can be violated. The 
type-id is generated statically and there is no way to prevent an 
attacker from re-using a legitimate dangling pointer. Thus, none of the 
existing literature utilizing PAC fulfills all 3 properties.


==> _design.tex <==
\section{\sys Design}
\label{s:design}

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figs/properties}

	\caption{
    %
	Violations of three security properties on a pointer.
    %
	}

	\label{f:prop}
\end{figure}

%#### PACTight design
% - brief intro to sections
In this section, we will discuss our goals that we wish to achieve to
overcome the limitations of previous PAC approaches, the security
properties that should be enforced to achieve these goals, and
\sys's design overview and mechansim.

% #### PACTight goals
% - Introduce the goals we want based on the limitations discussed in 2.3
% - Formally list the goals that are required with description
\subsection{\sys goals}
\label{s:design:goals}

\MI{I am not sure if I should mention sensitive pointers here or not, and whether
or not I should mention "\sys's scheme" since it wasn't discussed. I don't want to
fall in the same generalization trap we fell into with VIP.}
\AQ{Maybe can word it like: Thus, we choose to implement \sys-CPI to protect...
in order to make it more clear \sys is just pointer protection scheme, and \sys-CPI
uses that scheme to protect sens pointers.}
Based on the limitations we discussed in ~\autoref{s:bg:attack}, we identified
several goals that need to be achieved in order to overcome them. We believe
that achieving these goals would completely enforce pointer integrity
and prevent any pointer misuse. In addition to that, the defense mechanisms
implemented should have a low performance overhead. As with any scheme, naive use
of \sys's scheme could result in high overhead. Thus, we choose to implement \sys's
scheme to protect sensitive pointers ~\cite{kuznetsov:cpi}. Sensitive pointers are all
code pointers and pointers that point to code pointers. Our choice is due to that
protecting these sensitive pointers with \sys's scheme \emph{guarantees the integrity
of all sensitive pointers in a program}, completely preventing control-flow hijack attacks
in the program, and provide precise, deterministic memory safety for these sensitive
pointers. We discuss and elaborate more on our defense mechanisms in ~\autoref{s:defense}.
Thus, our main goals are:
\begin{itemize}[leftmargin=*]
%
\item Prevent any misuse of corrupted sensitive pointers.
%
%\item A sensitive pointer cannot be forged. Thus, a pointer
%\cc{p} should always point to its legitimate object.
%
%\item A sensitive pointer cannot be copied maliciously. Thus,
%a pointer \cc{p} can only be used when it is at it's specific location.
%
%\item A sensitive pointer cannot be abused in temporal attacks.
%Thus, a pointer \cc{p} cannot be used after it has been freed.
%
\item Compatibility with legacy C/C++ programs.
%
\item Low runtime and memory overhead.
%
\end{itemize}

%#### PACTight security properties
% Figures: Figures of the three properties
% - Introduce the three security properties based on the goals
% - Full description of the three properties
% - Why these three properties and their importance?
\subsection{\sys security properties}
\label{s:design:prop}

Based on the limitations of prior PAC approaches that we discussed in
~\autoref{s:bg:attack} and our goals in ~\autoref{s:design:goals}, we
define three security properties that, if achieved, would prevent
any misuse of pointers. These properties can be generalized to all
pointers, or to a specific subset of pointers. As mentioned before, we
focus on sensitive pointers in this work. These properties are:

\begin{enumerate}[leftmargin=*]
%
\item Unforgeability: A pointer cannot be forged. Thus, a
pointer \cc{p} should always point to its legitimate object.
%
\item Non-copyability: A pointer cannot be copied maliciously. Thus,
a pointer \cc{p} can only be used when it is at it's specific location.
%
\item Non-dangling: A pointer cannot be abused in temporal attacks.
Thus, a pointer \cc{p} cannot be used after it has been freed.
%
\end{enumerate}

~\autoref{f:props} showcases these properties and what violations of
them are like. Thus, in order to achieve the three properties, the design
has to prevent any of these violations from happening to its targeted type
of pointers.

\pp{Why these three properties?}
\YJ{Yes, prop 1 asserts that only generated pointer via PAC can be used.
prop 2 asserts that a live pointer can be referred only from a correct location.
so it prevents re-use of live poitners.
prop 3 asserts that a dead pointer cannot be re-used.}
\AQ{I might not be thinking about this correctly, but prop 2 to me seems
like preventing re-use and not spatial safety. Our spatial safety derives
from the hashtable and the inability to forge pointers that are OOB.}
The importance of these properties stems from the fact that
in order to hijack control-flow, at least one of these properties must be
violated. This is due to the definition of a control-flow hijack attack.
A control-flow hijack attack involves subverting the control-flow of the
program by \emph{altering a code pointer (\ie, influencing the program counter)
or changing a memory region that should not be accessed}. Property 1 and
property 2 tightly seal a code pointer and prevent any alterations to it.
Property 3 handles the unauthorized access of a freed memory region (\ie
a region that should not be accessed). Bear in mind that property 2 handles
spatial safety (\emph{a pointer \cc{p} can only be used when it is at
it's specific location.}), and thus out-of-bounds accesses violate property 2.
Thus, these three properties tightly seal the pointers and prevent any
misuse of the pointers.

%#### PACTight design overview
% - PACTight high level design diagram
% - Introduce overall design based on achieving the three properties
% - Achieve them based on the PAC modifier
% - Show how this design will enforce the three properties
\subsection{\sys design overview}
\label{s:design:overview}

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\textwidth]{figs/pactight-arch2}
	\caption{\sys compile and runtime mechanism}
	\label{f:mech}
\end{figure*}

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figs/pactight-sign}

    \caption{
    %
    Signing and authentication of a pointer variable \cc{p} in \sys. In
    addition to unforgeability of \cc{p} provided by PA, \sys uses the address
    of a pointer (\cc{\&p}) and a random tag of a pointee (\cc{tag(p)}) to
    provide non-copiability and non-dangling properties of a \sys-signed
    pointer.
    %
    }

	\label{f:meta}
\end{figure}


In this section, we present a high-level overview of \sys, our novel
design for enforcing the three security properties. \sys is composed of
an LLVM instrumentation pass to detect all the pointers that need to be
sealed. It also consists of a runtime library, integrated into the
LLVM compiler\_rt. The library protects the identified pointers with
our own unique mechanism based on PAC. ~\autoref{f:design} shows a high
level overview.

\pp{Enforcing the three properties}
In order to enforce the three properties, \sys relies on the modifier
in PAC. The modifier is a user-defined salt that is incorporated by
the cryptographic algorithm into the PAC. Any change to it would
result in a different PAC. \sys incorporates all three security
properties into the modifier. This means that any violation of any
one security property would be detected. We propose a complex modifier
of both static and dynamic elements.

\begin{itemize}[leftmargin=*]
%
\item Unforgeability: PAC's mechanism includes the pointer
as part of the PAC. Thus, this achieves the first property
to make the pointer unforgeable.
%
\item Non-copyability: \sys adds the location of the
pointer (\&p) as part of the modifier. This guarantees that
the pointer can only be used at that specific location. Any
change in the location by copying the pointer would change
the modifier and thus trigger an authentication fault.
%
\item Non-dangling: \sys adds dynamic metadata that is
defined upon allocation and deleted upon deallocation. This
is done for both the stack and the heap. This means that if
a pointer is getting used outside of its legitimate window
between allocation and deallocation, there will be no metadata
and \sys detects it.
%
\end{itemize}

By incorporating all these information together into the modifier,
\sys is able to generate a complex and unique modifier. All the
information used is reproducable at both the signing and
authenticating of the pointer. As mentioned before, any change
to any of this information changes the modifier, which changes
the PAC, and thus authentication would fail.


%#### PACTight mechanism
% Figures: PACTight runtime code snippets and PACTight metadata
% - Explain runtime
% - PACTight metadata
% - Discuss hashtable implications
\subsection{\sys mechanism}
\label{s:design:mechanism}

In this section we describe in detail how \sys's runtime
mechanism works, and the metadata design and it's implications.

\pp{\sys runtime}
\sys's library is integrated within the LLVM framework in compiler\_rt.
Thus, there is no need to include a shared library. The library
contains functions to:
\begin{itemize}[leftmargin=*]
%
\item Set the metadata for each pointer (\cc{setMetadata}).
%
\item Retrieve the metadata, build the modifier and add the PAC
to the pointer (\cc{addPAC}).
%
\item Retrieve the metadata, build the modifier and authenticate
the PAC on the pointer (\cc{authenticatePAC}).
%
\item Delete the metadata from memory (\cc{removeMetadata}).
%
\end{itemize}

\autoref{f:mech} shows how \sys's mechanism works.
When a pointer gets allocated, \cc{setMetadata} from the runtime
library allocates the metadata, sets a random token and all the
associated metadata. The number of elements and type size can be
determined statically by analyzing the LLVM IR. If it is a local
stack variable, only \cc{setMetadata} is called, since the pointer
still hasn't been assigned. If it is a heap variable (malloced)
then the metadata is set (\cc{setMetadata}) and the PAC is added
(\cc{addPAC}). Whenever the stack variable is assigned, the PAC
is added with \cc{addPAC}. In case of arrays, each element in the
array gets a unique random token, with the rest of the metadata
keeping track of the number of elements in the array.

If any change in assignment happens to the pointer legitimately,
the PAC is authenticated (\cc{authPAC}) and a new PAC is generated
for the new pointer with \cc{addPAC}.

%\sys handles special cases, such as \cc{memcpy}
%and \cc{munmap}, separately with its own intrinsics. Since they
%have void\* arguments, \sys gets the actual operand type first and
%instrumentation is done accordingly. This is not only
%done for \cc{memcpy} and \cc{munmap}, but for all universal pointers.
%\sys looks ahead for its typecasting and instrumentation is done
%accordingly as well.

When a pointer gets deallocated, the pointer is authenticated and all
metadata is removed (\emph{removeMetadata}). This is done by
reading the type size and no. of elements from the metadata and
removing the metadata accordingly. This prevents the metadata
from being reused by the attacker.

%%
\pp{\sys Metadata Design}
%
\sys adds a dynamic aspect to the modifier by
using a lightweight metadata composed of three main
elements:
%
\begin{itemize}[leftmargin=*]
%
\item A random token: This is a random 8-byte token
generated at random upon allocation.
%
\item Number of elements: This keeps track of the number
of elements allocated by this specific object, for
example, in case of a an array allocation.
%
\item Type size: This keeps track of the size
of each individual element.
%
\end{itemize}
%
The reason we use a random token is to add an aspect of randomness to the
modifier, and the use of a random token allows us to change the modifier
easily if another pointer of the same type gets reallocated at the same
memory location. Thus, we can always guarantee that the modifier is unique
and thus the PAC will always be unique, even for the same pointer type at
the same location. The number of elements and type size allow the metadata
to be revoked accordingly upon deallocation, since freeing the object may
be done independently from where the object was first allocated.
The revocation of the metadata means that if the attacker tries
to reuse a dangling PACed pointer, there would be no corresponding
metadata. \sys detects this and immediately halts the
program. Any change to the random token would also be detected
by \sys. The metadata itself contains no discernable
information to the attacker i.e - no pointer addresses. Thus, it
is probabilistically harder for the attacker to exploit it.

\AQ{I think our scheme should concat rather than XOR so metadata
corruption doesn't violate prop 2.}
\YJ{We should use blend}
~\autoref{f:meta} shows how \sys's protection scheme for generating
the PAC works. The location of the pointer (\&p) and the random token
are XOR'ed together, and these form the modifier passed to the PA
instruction. Thus, the PAC generated has the pointer, location of
the pointer, a random token and the key included in the modifier.
This forms a strong and extremely unique modifer. When the PAC is
generated and added to the pointer, the pointer now achieves all
3 security properties discussed above. \sys relies on its
runtime library to control the metadata (initialize, set and remove)
, add the PACs and authenticate the PACs.



\if 0
\CM{This section is the key of this paper. It should be at least 3 pages.
Please describe why and how to in detail.}

\MI{Figure 3: \sys metadata design. Figure 4: \sys compile time and runtime use.}
\MI{Figure 5 - \sys architecture (Diagram similar PARTS diagram 3)}

\subsection{\sys} \CM{If a section has only one subsection, that subsection
would be better to be merged to the section.}
\label{s:design:pactight}


\CM{Fig 3, 4, 5 are not referenced in the text. You should present figures in
a top-down manner; You should present a high level overview introducing the
components in \sys first then presents more details as you describe the
details. But fig 3 is the most detailed and fig 4 and 5 look high level design.
Also, it is not clear how fig 4 and fig 4 are different. }

\CM{
Somewhere in the design section, you should discuss the security implication of
using a large hash table. Entropy is of course low and an attacker can corrupt
it. Is that still safe? What's our assumption and counter arguments on that?
}

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figs/pactight-metadata}

    \caption{\sys  metadata design.
    %
    \CM{
    - Add a period at the end of the caption.
    - Readers will be able to how this diagram matches with Fig 1 and 2.
    - You need to clearly present what PAC provides and what \sys provides in
    the diagram.
    }
    %
    }

	\label{f:meta}
\end{figure}

\begin{figure*}[t]
	\noindent
	\includegraphics[width=\textwidth]{figs/pactight-mechanism}
	\caption{
		\textbf{\sys compile and runtime mechanism}
	}
%	\vspace{-1.5em}
	\label{f:mech}
\end{figure*}

\CM{
%
- Rewrite this section.
- You explained only HOW \sys works. But more important one is WHY it should
be. For example, you should explain why you decided to use a random tag and how
using a random tag helps to achieve three properties and our goal altogether.
- It is hard for reviewers to discover your novelty and significance if you
do not explain WHY.
%
}

Our main goals aim to achieve security against
control-flow hijacking and temporal attacks against
sensitive pointers, in addition to preventing the
reuse of PACs. Thus, our design for \sys aims
to achieve this.

%%
\pp{\sys Metadata Design}
%
\sys adds a dynamic aspect to the modifier by
using a lightweight metadata composed of three main
elements:
%
\begin{itemize}[leftmargin=*]
%
\item A random token: This is a random 8-byte token
generated at random upon allocation.
%
\item \XXX{No.}\CM{Avoid to use contractions.}
of elements: This keeps track of the number
of elements allocated by this specific object, for
example, in case of a an array allocation.
%
\item Type size: This keeps track of the size
of each individual element.
%
\end{itemize}
%
\AQ{The claim that it is probablistically harder for an attacker
to exploit needs to be more clear or removed. Are you saying that
the attacker does not know which entry corresponds to which pointer?
The hash function is public so this is not the case. An attacker can
look at the area he thinks is the hashtable before alloc, then after
alloc, find where the entry got added, find what the pointer hashes to,
then subtract the two to figure out the hashtable base.}
The no. of elements and type size allow the metadata
to be revoked accordingly upon deallocation, since freeing the object may
be done independently from where the object was first allocated.
The revocation of the metadata means that if the attacker tries
to reuse a dangling PACed pointer, there would be no corresponding
metadata. \sys detects this and immediately halts the
program. Any change to the random token would also be detected
by \sys. The metadata itself contains no discernable
information to the attacker i.e - no pointer addresses. Thus, it
is probabilistically harder for the attacker to exploit it.

~\autoref{f:meta} shows how \sys's protection scheme for generating
the PAC works. The location of the pointer (\&p) and the random token
are XOR'ed together, and these form the modifier passed to the PA
instruction. Thus, the PAC generated has the pointer, location of
the pointer, a random token and the key included in the modifier.
This forms a strong and extremely unique modifer. When the PAC is
generated and added to the pointer, the pointer now achieves all
3 security properties discussed above. \sys relies on its
runtime library to control the metadata (initialize, set and remove)
, add the PACs and authenticate the PACs.

%%
\pp{\sys Security Properties} \CM{
%
This should be first explained before explaining how \sys works. That way you
can explain how your techniques helps to achieve three properties.
%
}
%
In order to achieve the main goals, we believe an inherently
unique modifier is key to the design. Thus, we propose a
complex modifier of both static and dynamic elements to achieve
all three properties discussed earlier.
%
\begin{itemize}[leftmargin=*]
%
\item Unforgeability: PA's mechanism includes the pointer
as part of the PAC. Thus, this achieves the first property
to make the pointer unforgeable.
%
\item Non-copyability: \sys adds the location of the
pointer (\&p) as part of the modifier. This guarantees that
the pointer can only be used at that specific location. Any
change in the location by copying the pointer would change
the modifier and thus trigger an authentication fault.
%
\item Non-dangling: \sys adds dynamic metadata that is
defined upon allocation and deleted upon deallocation. This
is done for both the stack and the heap. This means that if
a pointer is getting used outside of its legitimate window
between allocation and deallocation, there will be no metadata
and \sys detects it.
%
\end{itemize}
%
\fi


==> _intro.tex <==
\tsection{Introduction}
\label{s:intro}

% ARM is getting popular!
In the past few years, there has been an increase in popularity and attention
to the ARMv8 processor architecture, particularly in its use in desktops and
data centers. Several vendors, including Apple ~\cite{apple:m1},
Oracle~\cite{oracle:arm} and Qualcomm~\cite{qualcomm:arm}, have shown and
invested into the technology. As it becomes more advanced and sophisticated, so
well the possible attacks against it. Thus, it has become more important to
develop defences for this architecture against complex attacks.

% [?] Attacks: memory corruption, code injection, DEP, CFI, CPI
Memory corruption attacks are some of the most common attacks against software.
Since C and C++ are unsafe languages, it is easy for an attacker to violate the
the language rules. This has led to attacks such as code injection and
control-flow hijacking attacks. Code injection is no longer possible due to the
universal enforcement of Data Execution Prevention (DEP). However, control-flow
hijacking attacks are still prevalent. These attacks aim to subvert the
control-flow of a program by carefully corrupting code pointers, such as return
addresses and function pointers. Control-flow integrity (CFI) ~\cite{cfi} aims
to defend against these attacks by ensuring the program follows its proper
control-flow. This is mainly done by computing a control-flow graph (CFG) and
conforming to it. Most CFI techniques are either efficient but imprecise
(coarse-grained) or precise but inefficient (fine-grained). Code Pointer
Integrity (CPI) ~\cite{kuznetsov:cpi} aims to protect against control-flow
hijacking by guaranteeing the integrity of code pointers in a program. CPI
defends by isolating these code pointers in a disjoint metadata. However, CPI
doesn't defend against temporal attacks against these code pointers, and has
high memory overhead (105\% on average) to keep track of all the metadata. 

% ARM PA: new, promising hardware security feature
ARM has introduced several hardware security features to defend against memory
corruption attacks. One of these is \emph{Pointer Authentication (PA)},a
security feature that is intended to ensure pointer integrity with
cryptographic primitives. PA computes a cryptographic MAC called a Pointer
Authentication Code (PAC) and stores it in the upper bits of the 64-bit
pointer. PA can be used to defend against control-flow hijacking attacks
securely and efficiently. Its hardware implementation and use of the unused
bits in the 64-bit address give it the ability to achieve a low performance and
memory overhead. 

% weaknesses of prior ARM PA based defenses
However, PA isn't without its limitations. It can be exposed to attacks if it
is used naively. Moreover, recent mechanisms that utilize
PA~\cite{parts-lilijestrand-sec19, pacstack-lilijestrand-sec21,
pcan-lilijestrand-systex19, ptauth-farkhani-sec21, apple:pac, qualcomm:pac}
have weaknesses that can still expose them to attacks, such as using a signing
gadget to forge PACs~\cite{google:pac}, and reusing of PACs that have the same
modifier~\cite{parts-lilijestrand-sec19}. In spite of the fact that the main
motivation behind PAC is to secure pointers to prevent pointer attacks, the
attacks may still occur.

% [?] modifier, the source of all weakness
Our observation in these limitations and attacks is that these mechanisms
are exposed to pointer integrity attacks due to a weak modifier. If the modifier
is strong enough, then the PAC is unique and can't be abused. The choice of the 
modifier must be carefully designed to protect against all possible methods that
can tamper with the pointer and subvert its control flow. Our goal is to achieve 
this design and completely prevent pointers from being tampered with (\ie sealed).

% our analysis: three properties
Based on the limitations and our goal, we define three security properties
that, if achieved, prevent pointers from being tampered with.
1) Unforegablity: A pointer \emph{p} should always point to its legitimate
object. 2) Non-copyability: A pointer \emph{p} can only be used when it is at
it's specific legitimate location. 3) Non-dangling: A pointer \emph{p} cannot
be used after it has been freed.

% pactight
Thus we propose, \sys, our novel and efficient scheme to guarantee all
3 properties: unforegable, non-copyable and non-dangling pointers. \sys tightly
seals pointers with fine grained protection using a PAC generated with a strong
and unique modifier. Our modifier has both static and dynamic properties
incorporated in it. \sys provides guarantees that pointers cannot be forged,
copied, and are not dangling.

% goal, scope, defenses
We focus implementing \sys to achieve pointer integrity by protecting all
sensitive pointers and provide precise, deterministic memory safety for these
sensitive pointers. Sensitive pointers are all code pointers and data pointers
that point to code pointers. Protecting these sensitive pointers achieves the
balance for reinforced protection, thus achieving protection against
control-flow hijacking attacks and providing memory safety for sensitive
pointers. 
%
We provide many implementations of \sys: \sys-Stack protects all return
addresses from ROP, \sys-CFI-VTable protects all forward-edge and backward-edge
control flow transfers, in addition to all VTable pointers in C++, \sys-CPI
protects all the above in addition to a subset of data pointers, particularly
pointers to code pointers.

% summary
Thus our contributions are:
\squishlists

\item \sys: a novel and efficient approach to tightly seal pointers, and
achieve a pointer that is unforgeable, non-copyable, and non-dangling.

\item We provide three implementations of our \sys scheme: \sys-CFI,
\sys-VTable, \sys-CPI, and \sys return address protection.

\item We provide a strong security evaluation by analysing our scheme,
demonstrate effectiveness against real-world CVEs and synthesised attacks.

\item We evaluate \sys implementations on SPEC2006 benchmarks and NGINX web
server. We show that \sys implementations achieve low performance overhead
making it possible to implement \sys schemes in the real-world.

\squishends



==> bin/latexrun <==
#!/usr/bin/env python3

# Copyright (c) 2013, 2014 Austin Clements

# Permission is hereby granted, free of charge, to any person obtaining a copy
# of this software and associated documentation files (the "Software"), to deal
# in the Software without restriction, including without limitation the rights
# to use, copy, modify, merge, publish, distribute, sublicense, and/or sell
# copies of the Software, and to permit persons to whom the Software is
# furnished to do so, subject to the following conditions:

# The above copyright notice and this permission notice shall be included in
# all copies or substantial portions of the Software.

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
# IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
# FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN NO EVENT SHALL THE
# AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER
# LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM,
# OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN
# THE SOFTWARE.

import sys
import os
import errno
import argparse
import shlex
import json
import subprocess
import re
import collections
import hashlib
import shutil
import curses
import filecmp
import io
import traceback
import time

try:
    import fcntl
except ImportError:
    # Non-UNIX platform
    fcntl = None

def debug(string, *args):
    if debug.enabled:
        print(string.format(*args), file=sys.stderr)
debug.enabled = False

def debug_exc():
    if debug.enabled:
        traceback.print_exc()

def main():
    # Parse command-line
    arg_parser = argparse.ArgumentParser(
        description='''A 21st century LaTeX wrapper,
        %(prog)s runs latex (and bibtex) the right number of times so you
        don't have to,
        strips the log spew to make errors visible,
        and plays well with standard build tools.''')
    arg_parser.add_argument(
        '-o', metavar='FILE', dest='output', default=None,
        help='Output file name (default: derived from input file)')
    arg_parser.add_argument(
        '--latex-cmd', metavar='CMD', default='pdflatex',
        help='Latex command (default: %(default)s)')
    arg_parser.add_argument(
        '--latex-args', metavar='ARGS', type=arg_parser_shlex,
        help='Additional command-line arguments for latex.'
        ' This will be parsed and split using POSIX shell rules.')
    arg_parser.add_argument(
        '--bibtex-cmd', metavar='CMD', default='bibtex',
        help='Bibtex command (default: %(default)s)')
    arg_parser.add_argument(
        '--bibtex-args', metavar='ARGS', type=arg_parser_shlex,
        help='Additional command-line arguments for bibtex')
    arg_parser.add_argument(
        '--max-iterations', metavar='N', type=int, default=10,
        help='Max number of times to run latex before giving up'
        ' (default: %(default)s)')
    arg_parser.add_argument(
        '-W', metavar='(no-)CLASS',
        action=ArgParserWarnAction, dest='nowarns', default=set(['underfull']),
        help='Enable/disable warning from CLASS, which can be any package name, '
        'LaTeX warning class (e.g., font), bad box type '
        '(underfull, overfull, loose, tight), strict parsing (strict-parse),  or "all"')
    arg_parser.add_argument(
        '-O', metavar='DIR', dest='obj_dir', default='latex.out',
        help='Directory for intermediate files and control database '
        '(default: %(default)s)')
    arg_parser.add_argument(
        '--color', choices=('auto', 'always', 'never'), default='auto',
        help='When to colorize messages')
    arg_parser.add_argument(
        '--verbose-cmds', action='store_true', default=False,
        help='Print commands as they are executed')
    arg_parser.add_argument(
        '--debug', action='store_true',
        help='Enable detailed debug output')
    actions = arg_parser.add_argument_group('actions')
    actions.add_argument(
        '--clean-all', action='store_true', help='Delete output files')
    actions.add_argument(
        'file', nargs='?', help='.tex file to compile')
    args = arg_parser.parse_args()
    if not any([args.clean_all, args.file]):
        arg_parser.error('at least one action is required')
    args.latex_args = args.latex_args or []
    args.bibtex_args = args.bibtex_args or []

    verbose_cmd.enabled = args.verbose_cmds
    debug.enabled = args.debug

    # A note about encodings: POSIX encoding is a mess; TeX encoding
    # is a disaster.  Our goal is to make things no worse, so we want
    # byte-accurate round-tripping of TeX messages.  Since TeX
    # messages are *basically* text, we use strings and
    # surrogateescape'ing for both input and output.  I'm not fond of
    # setting surrogateescape globally, but it's far easier than
    # dealing with every place we pass TeX output through.
    # Conveniently, JSON can round-trip surrogateescape'd strings, so
    # our control database doesn't need special handling.
    sys.stdout = io.TextIOWrapper(
        sys.stdout.buffer, encoding=sys.stdout.encoding,
        errors='surrogateescape', line_buffering=sys.stdout.line_buffering)
    sys.stderr = io.TextIOWrapper(
        sys.stderr.buffer, encoding=sys.stderr.encoding,
        errors='surrogateescape', line_buffering=sys.stderr.line_buffering)

    Message.setup_color(args.color)

    # Open control database.
    dbpath = os.path.join(args.obj_dir, '.latexrun.db')
    if not os.path.exists(dbpath) and os.path.exists('.latexrun.db'):
        # The control database used to live in the source directory.
        # Support this for backwards compatibility.
        dbpath = '.latexrun.db'
    try:
        db = DB(dbpath)
    except (ValueError, OSError) as e:
        print('error opening {}: {}'.format(e.filename if hasattr(e, 'filename')
                                            else dbpath, e),
              file=sys.stderr)
        debug_exc()
        sys.exit(1)

    # Clean
    if args.clean_all:
        try:
            db.do_clean(args.obj_dir)
        except OSError as e:
            print(e, file=sys.stderr)
            debug_exc()
            sys.exit(1)

    # Build
    if not args.file:
        return
    task_commit = None
    try:
        task_latex = LaTeX(db, args.file, args.latex_cmd, args.latex_args,
                           args.obj_dir, args.nowarns)
        task_commit = LaTeXCommit(db, task_latex, args.output)
        task_bibtex = BibTeX(db, task_latex, args.bibtex_cmd, args.bibtex_args,
                             args.nowarns, args.obj_dir)
        tasks = [task_latex, task_commit, task_bibtex]
        stable = run_tasks(tasks, args.max_iterations)

        # Print final task output and gather exit status
        status = 0
        for task in tasks:
            status = max(task.report(), status)

        if not stable:
            print('error: files are still changing after {} iterations; giving up'
                  .format(args.max_iterations), file=sys.stderr)
            status = max(status, 1)
    except TaskError as e:
        print(str(e), file=sys.stderr)
        debug_exc()
        status = 1

    # Report final status, if interesting
    fstatus = 'There were errors' if task_commit is None else task_commit.status
    if fstatus:
        output = args.output
        if output is None:
            if task_latex.get_outname() is not None:
                output = os.path.basename(task_latex.get_outname())
            else:
                output = 'output'
        if Message._color:
            terminfo.send('bold', ('setaf', 1))
        print('{}; {} not updated'.format(fstatus, output))
        if Message._color:
            terminfo.send('sgr0')
    sys.exit(status)

def arg_parser_shlex(string):
    """Argument parser for shell token lists."""
    try:
        return shlex.split(string)
    except ValueError as e:
        raise argparse.ArgumentTypeError(str(e)) from None

class ArgParserWarnAction(argparse.Action):
    def __call__(self, parser, namespace, value, option_string=None):
        nowarn = getattr(namespace, self.dest)
        if value == 'all':
            nowarn.clear()
        elif value.startswith('no-'):
            nowarn.add(value[3:])
        else:
            nowarn.discard(value)
        setattr(namespace, self.dest, nowarn)

def verbose_cmd(args, cwd=None, env=None):
    if verbose_cmd.enabled:
        cmd = ' '.join(map(shlex.quote, args))
        if cwd is not None:
            cmd = '(cd {} && {})'.format(shlex.quote(cwd), cmd)
        if env is not None:
            for k, v in env.items():
                if os.environ.get(k) != v:
                    cmd = '{}={} {}'.format(k, shlex.quote(v), cmd)
        print(cmd, file=sys.stderr)
verbose_cmd.enabled = False

def mkdir_p(path):
    try:
        os.makedirs(path)
    except OSError as exc:
        if exc.errno == errno.EEXIST and os.path.isdir(path):
            pass
        else: raise

def nested_parenthesis_end(string, opening, closing, lax_checking=False):
    """Return index where closing character corresponds to opening character"""
    stack = []
    for i, c in enumerate(string):
        if c in opening:
            stack.append(c)
        elif c in closing and stack:
            start_ch = stack.pop()
            if not lax_checking and opening.index(start_ch) != closing.index(c):
                # Mismatch, e.g. expected ')', found '}'
                return -1
            if not stack:
                return i
    return -1

class DB:
    """A latexrun control database."""

    _VERSION = 'latexrun-db-v2'

    def __init__(self, filename):
        self.__filename = filename

        try:
            fp = open(filename, 'r')
        except FileNotFoundError:
            debug('creating new database')
            self.__val = {'version': DB._VERSION}
        else:
            debug('loading database')
            self.__val = json.load(fp)
            if 'version' not in self.__val:
                raise ValueError('file exists, but does not appear to be a latexrun database'.format(filename))
            if self.__val['version'] != DB._VERSION:
                raise ValueError('unknown database version {!r}'
                                 .format(self.__val['version']))

    def commit(self):
        debug('committing database')
        # Make sure database directory exists
        if os.path.dirname(self.__filename):
            os.makedirs(os.path.dirname(self.__filename), exist_ok=True)
        # Atomically commit database
        tmp_filename = self.__filename + '.tmp'
        with open(tmp_filename, 'w') as fp:
            json.dump(self.__val, fp, indent=2, separators=(',', ': '))
            fp.flush()
            os.fsync(fp.fileno())
        os.rename(tmp_filename, self.__filename)

    def get_summary(self, task_id):
        """Return the recorded summary for the given task or None."""
        return self.__val.get('tasks', {}).get(task_id)

    def set_summary(self, task_id, summary):
        """Set the summary for the given task."""
        self.__val.setdefault('tasks', {})[task_id] = summary

    def add_clean(self, filename):
        """Add an output file to be cleaned.

        Unlike the output files recorded in the task summaries,
        cleanable files strictly accumulate until a clean is
        performed.
        """
        self.__val.setdefault('clean', {})[filename] = hash_cache.get(filename)

    def do_clean(self, obj_dir=None):
        """Remove output files and delete database.

        If obj_dir is not None and it is empty after all files are
        removed, it will also be removed.
        """

        for f, want_hash in self.__val.get('clean', {}).items():
            have_hash = hash_cache.get(f)
            if have_hash is not None:
                if want_hash == have_hash:
                    debug('unlinking {}', f)
                    hash_cache.invalidate(f)
                    os.unlink(f)
                else:
                    print('warning: {} has changed; not removing'.format(f),
                          file=sys.stderr)
        self.__val = {'version': DB._VERSION}
        try:
            os.unlink(self.__filename)
        except FileNotFoundError:
            pass
        if obj_dir is not None:
            try:
                os.rmdir(obj_dir)
            except OSError:
                pass

class HashCache:
    """Cache of file hashes.

    As latexrun reaches fixed-point, it hashes the same files over and
    over, many of which never change.  Since hashing is somewhat
    expensive, we keep a simple cache of these hashes.
    """

    def __init__(self):
        self.__cache = {}

    def get(self, filename):
        """Return the hash of filename, or * if it was clobbered."""
        try:
            with open(filename, 'rb') as fp:
                st = os.fstat(fp.fileno())
                key = (st.st_dev, st.st_ino)
                if key in self.__cache:
                    return self.__cache[key]

                debug('hashing {}', filename)
                h = hashlib.sha256()
                while True:
                    block = fp.read(256*1024)
                    if not len(block):
                        break
                    h.update(block)
                self.__cache[key] = h.hexdigest()
                return self.__cache[key]
        except (FileNotFoundError, IsADirectoryError):
            return None

    def clobber(self, filename):
        """If filename's hash is not known, record an invalid hash.

        This can be used when filename was overwritten before we were
        necessarily able to obtain its hash.  filename must exist.
        """
        st = os.stat(filename)
        key = (st.st_dev, st.st_ino)
        if key not in self.__cache:
            self.__cache[key] = '*'

    def invalidate(self, filename):
        try:
            st = os.stat(filename)
        except OSError as e:
            # Pessimistically wipe the whole cache
            debug('wiping hash cache ({})', e)
            self.__cache.clear()
        else:
            key = (st.st_dev, st.st_ino)
            if key in self.__cache:
                del self.__cache[key]
hash_cache = HashCache()

class _Terminfo:
    def __init__(self):
        self.__tty = os.isatty(sys.stdout.fileno())
        if self.__tty:
            curses.setupterm()
        self.__ti = {}

    def __ensure(self, cap):
        if cap not in self.__ti:
            if not self.__tty:
                string = None
            else:
                string = curses.tigetstr(cap)
                if string is None or b'$<' in string:
                    # Don't have this capability or it has a pause
                    string = None
            self.__ti[cap] = string
        return self.__ti[cap]

    def has(self, *caps):
        return all(self.__ensure(cap) is not None for cap in caps)

    def send(self, *caps):
        # Flush TextIOWrapper to the binary IO buffer
        sys.stdout.flush()
        for cap in caps:
            # We should use curses.putp here, but it's broken in
            # Python3 because it writes directly to C's buffered
            # stdout and there's no way to flush that.
            if isinstance(cap, tuple):
                s = curses.tparm(self.__ensure(cap[0]), *cap[1:])
            else:
                s = self.__ensure(cap)
            sys.stdout.buffer.write(s)
terminfo = _Terminfo()

class Progress:
    _enabled = None

    def __init__(self, prefix):
        self.__prefix = prefix
        if Progress._enabled is None:
            Progress._enabled = (not debug.enabled) and \
                                terminfo.has('cr', 'el', 'rmam', 'smam')

    def __enter__(self):
        self.last = ''
        self.update('')
        return self

    def __exit__(self, typ, value, traceback):
        if Progress._enabled:
            # Beginning of line and clear
            terminfo.send('cr', 'el')
            sys.stdout.flush()

    def update(self, msg):
        if not Progress._enabled:
            return
        out = '[' + self.__prefix + ']'
        if msg:
            out += ' ' + msg
        if out != self.last:
            # Beginning of line, clear line, disable wrap
            terminfo.send('cr', 'el', 'rmam')
            sys.stdout.write(out)
            # Enable wrap
            terminfo.send('smam')
            self.last = out
            sys.stdout.flush()

class Message(collections.namedtuple(
        'Message', 'typ filename lineno msg')):
    def emit(self):
        if self.filename:
            if self.filename.startswith('./'):
                finfo = self.filename[2:]
            else:
                finfo = self.filename
        else:
            finfo = '<no file>'
        if self.lineno is not None:
            finfo += ':' + str(self.lineno)
        finfo += ': '
        if self._color:
            terminfo.send('bold')
        sys.stdout.write(finfo)

        if self.typ != 'info':
            if self._color:
                terminfo.send(('setaf', 5 if self.typ == 'warning' else 1))
            sys.stdout.write(self.typ + ': ')
        if self._color:
            terminfo.send('sgr0')
        sys.stdout.write(self.msg + '\n')

    @classmethod
    def setup_color(cls, state):
        if state == 'never':
            cls._color = False
        elif state == 'always':
            cls._color = True
        elif state == 'auto':
            cls._color = terminfo.has('setaf', 'bold', 'sgr0')
        else:
            raise ValueError('Illegal color state {:r}'.format(state))


##################################################################
# Task framework
#

terminate_task_loop = False
start_time = time.time()

def run_tasks(tasks, max_iterations):
    """Execute tasks in round-robin order until all are stable.

    This will also exit if terminate_task_loop is true.  Tasks may use
    this to terminate after a fatal error (even if that fatal error
    doesn't necessarily indicate stability; as long as re-running the
    task will never eliminate the fatal error).

    Return True if fixed-point is reached or terminate_task_loop is
    set within max_iterations iterations.
    """

    global terminate_task_loop
    terminate_task_loop = False

    nstable = 0
    for iteration in range(max_iterations):
        for task in tasks:
            if task.stable():
                nstable += 1
                if nstable == len(tasks):
                    debug('fixed-point reached')
                    return True
            else:
                task.run()
                nstable = 0
                if terminate_task_loop:
                    debug('terminate_task_loop set')
                    return True
    debug('fixed-point not reached')
    return False

class TaskError(Exception):
    pass

class Task:
    """A deterministic computation whose inputs and outputs can be captured."""

    def __init__(self, db, task_id):
        self.__db = db
        self.__task_id = task_id

    def __debug(self, string, *args):
        if debug.enabled:
            debug('task {}: {}', self.__task_id, string.format(*args))

    def stable(self):
        """Return True if running this task will not affect system state.

        Functionally, let f be the task, and s be the system state.
        Then s' = f(s).  If it must be that s' == s (that is, f has
        reached a fixed point), then this function must return True.
        """
        last_summary = self.__db.get_summary(self.__task_id)
        if last_summary is None:
            # Task has never run, so running it will modify system
            # state
            changed = 'never run'
        else:
            # If any of the inputs have changed since the last run of
            # this task, the result may change, so re-run the task.
            # Also, it's possible something else changed an output
            # file, in which case we also want to re-run the task, so
            # check the outputs, too.
            changed = self.__summary_changed(last_summary)

        if changed:
            self.__debug('unstable (changed: {})', changed)
            return False
        else:
            self.__debug('stable')
            return True

    def __summary_changed(self, summary):
        """Test if any inputs changed from summary.

        Returns a string describing the changed input, or None.
        """
        for dep in summary['deps']:
            fn, args, val = dep
            method = getattr(self, '_input_' + fn, None)
            if method is None:
                return 'unknown dependency method {}'.format(fn)
            if method == self._input_unstable or method(*args) != val:
                return '{}{}'.format(fn, tuple(args))
        return None

    def _input(self, name, *args):
        """Register an input for this run.

        This calls self._input_<name>(*args) to get the value of this
        input.  This function should run quickly and return some
        projection of system state that affects the result of this
        computation.

        Both args and the return value must be JSON serializable.
        """
        method = getattr(self, '_input_' + name)
        val = method(*args)
        if [name, args, val] not in self.__deps:
            self.__deps.append([name, args, val])
        return val

    def run(self):
        # Before we run the task, pre-hash any files that were output
        # files in the last run.  These may be input by this run and
        # then clobbered, at which point it will be too late to get an
        # input hash.  Ideally we would only hash files that were
        # *both* input and output files, but latex doesn't tell us
        # about input files that didn't exist, so if we start from a
        # clean slate, we often require an extra run because we don't
        # know a file is input/output until after the second run.
        last_summary = self.__db.get_summary(self.__task_id)
        if last_summary is not None:
            for io_filename in last_summary['output_files']:
                self.__debug('pre-hashing {}', io_filename)
                hash_cache.get(io_filename)

        # Run the task
        self.__debug('running')
        self.__deps = []
        result = self._execute()

        # Clear cached output file hashes
        for filename in result.output_filenames:
            hash_cache.invalidate(filename)

        # If the output files change, then the computation needs to be
        # re-run, so record them as inputs
        for filename in result.output_filenames:
            self._input('file', filename)

        # Update task summary in database
        self.__db.set_summary(self.__task_id,
                              self.__make_summary(self.__deps, result))
        del self.__deps

        # Add output files to be cleaned
        for f in result.output_filenames:
            self.__db.add_clean(f)

        try:
            self.__db.commit()
        except OSError as e:
            raise TaskError('error committing control database {}: {}'.format(
                getattr(e, 'filename', '<unknown path>'), e)) from e

    def __make_summary(self, deps, run_result):
        """Construct a new task summary."""
        return {
            'deps': deps,
            'output_files': {f: hash_cache.get(f)
                             for f in run_result.output_filenames},
            'extra': run_result.extra,
        }

    def _execute(self):
        """Abstract: Execute this task.

        Subclasses should implement this method to execute this task.
        This method must return a RunResult giving the inputs that
        were used by the task and the outputs it produced.
        """
        raise NotImplementedError('Task._execute is abstract')

    def _get_result_extra(self):
        """Return the 'extra' result from the previous run, or None."""
        summary = self.__db.get_summary(self.__task_id)
        if summary is None:
            return None
        return summary['extra']

    def report(self):
        """Report the task's results to stdout and return exit status.

        This may be called when the task has never executed.
        Subclasses should override this.  The default implementation
        reports nothing and returns 0.
        """
        return 0

    # Standard input functions

    def _input_env(self, var):
        return os.environ.get(var)

    def _input_file(self, path):
        return hash_cache.get(path)

    def _input_unstable(self):
        """Mark this run as unstable, regardless of other inputs."""
        return None

    def _input_unknown_input(self):
        """An unknown input that may change after latexrun exits.

        This conservatively marks some unknown input that definitely
        won't change while latexrun is running, but may change before
        the user next runs latexrun.  This allows the task to
        stabilize during this invocation, but will cause the task to
        re-run on the next invocation.
        """
        return start_time

class RunResult(collections.namedtuple(
        'RunResult', 'output_filenames extra')):
    """The result of a single task execution.

    This captures all files written by the task, and task-specific
    results that need to be persisted between runs (for example, to
    enable reporting of a task's results).
    """
    pass

##################################################################
# LaTeX task
#

def normalize_input_path(path):
    # Resolve the directory of the input path, but leave the file
    # component alone because it affects TeX's behavior.
    head, tail = os.path.split(path)
    npath = os.path.join(os.path.realpath(head), tail)
    return os.path.relpath(path)

class LaTeX(Task):
    def __init__(self, db, tex_filename, cmd, cmd_args, obj_dir, nowarns):
        super().__init__(db, 'latex::' + normalize_input_path(tex_filename))
        self.__tex_filename = tex_filename
        self.__cmd = cmd
        self.__cmd_args = cmd_args
        self.__obj_dir = obj_dir
        self.__nowarns = nowarns

        self.__pass = 0

    def _input_args(self):
        # If filename starts with a character the tex command-line
        # treats specially, then tweak it so it doesn't.
        filename = self.__tex_filename
        if filename.startswith(('-', '&', '\\')):
            filename = './' + filename
        # XXX Put these at the beginning in case the provided
        # arguments are malformed.  Might want to do a best-effort
        # check for incompatible user-provided arguments (note:
        # arguments can be given with one or two dashes and those with
        # values can use an equals or a space).
        return [self.__cmd] + self.__cmd_args + \
            ['-interaction', 'nonstopmode', '-recorder',
             '-output-directory', self.__obj_dir, filename]

    def _execute(self):
        # Run latex
        self.__pass += 1
        args = self._input('args')
        debug('running {}', args)
        try:
            os.makedirs(self.__obj_dir, exist_ok=True)
        except OSError as e:
            raise TaskError('failed to create %s: ' % self.__obj_dir + str(e)) \
                from e
        try:
            verbose_cmd(args)
            p = subprocess.Popen(args,
                                 stdin=subprocess.DEVNULL,
                                 stdout=subprocess.PIPE,
                                 stderr=subprocess.STDOUT)
            stdout, has_errors, missing_includes = self.__feed_terminal(p.stdout)
            status = p.wait()
        except OSError as e:
            raise TaskError('failed to execute latex task: ' + str(e)) from e

        # Register environment variable inputs
        for env_var in ['TEXMFOUTPUT', 'TEXINPUTS', 'TEXFORMATS', 'TEXPOOL',
                        'TFMFONTS', 'PATH']:
            self._input('env', env_var)

        jobname, outname = self.__parse_jobname(stdout)
        inputs, outputs = self.__parse_recorder(jobname)

        # LaTeX overwrites its own inputs.  Mark its output files as
        # clobbered before we hash its input files.
        for path in outputs:
            # In some abort cases (e.g., >=100 errors), LaTeX claims
            # output files that don't actually exist.
            if os.path.exists(path):
                hash_cache.clobber(path)
        # Depend on input files.  Task.run pre-hashed outputs from the
        # previous run, so if this isn't the first run and as long as
        # the set of outputs didn't change, we'll be able to get the
        # input hashes, even if they were clobbered.
        for path in inputs:
            self._input('file', path)

        if missing_includes:
            # Missing \includes are tricky.  Ideally we'd depend on
            # the absence of some file, but in fact we'd have to
            # depend on the failure of a whole kpathsea lookup.
            # Rather than try to be clever, just mark this as an
            # unknown input so we'll run at least once on the next
            # invocation.
            self._input('unknown_input')

        if not self.__create_outdirs(stdout) and has_errors:
            # LaTeX reported unrecoverable errors (other than output
            # directory errors, which we just fixed).  We could
            # continue to stabilize the document, which may change
            # some of the other problems reported (but not the
            # unrecoverable errors), or we can just abort now and get
            # back to the user quickly with the major errors.  We opt
            # for the latter.
            global terminate_task_loop
            terminate_task_loop = True
            # This error could depend on something we failed to track.
            # It would be really confusing if we continued to report
            # the error after the user fixed it, so be conservative
            # and force a re-run next time.
            self._input('unknown_input')

        return RunResult(outputs,
                         {'jobname': jobname, 'outname': outname,
                          'status': status})

    def __feed_terminal(self, stdout):
        prefix = 'latex'
        if self.__pass > 1:
            prefix += ' ({})'.format(self.__pass)
        with Progress(prefix) as progress:
            buf = []
            filt = LaTeXFilter()
            while True:
                # Use os.read to read only what's available on the pipe,
                # without waiting to fill a buffer
                data = os.read(stdout.fileno(), 4096)
                if not data:
                    break
                # See "A note about encoding" above
                data = data.decode('ascii', errors='surrogateescape')
                buf.append(data)
                filt.feed(data)
                file_stack = filt.get_file_stack()
                if file_stack:
                    tos = file_stack[-1]
                    if tos.startswith('./'):
                        tos = tos[2:]
                    progress.update('>' * len(file_stack) + ' ' + tos)
                else:
                    progress.update('')

            # Were there unrecoverable errors?
            has_errors = any(msg.typ == 'error' for msg in filt.get_messages())

            return ''.join(buf), has_errors, filt.has_missing_includes()

    def __parse_jobname(self, stdout):
        """Extract the job name and output name from latex's output.

        We get these from latex because they depend on complicated
        file name parsing rules, are affected by arguments like
        -output-directory, and may be just "texput" if things fail
        really early.  The output name may be None if there were no
        pages of output.
        """
        jobname = outname = None
        for m in re.finditer(r'^Transcript written on "?(.*)\.log"?\.$', stdout,
                             re.MULTILINE | re.DOTALL):
            jobname = m.group(1).replace('\n', '')
        if jobname is None:
            print(stdout, file=sys.stderr)
            raise TaskError('failed to extract job name from latex log')
        for m in re.finditer(r'^Output written on "?(.*\.[^ ."]+)"? \([0-9]+ page',
                             stdout, re.MULTILINE | re.DOTALL):
            outname = m.group(1).replace('\n', '')
        if outname is None and not \
           re.search(r'^No pages of output\.$|^! Emergency stop\.$'
                     r'|^!  ==> Fatal error occurred, no output PDF file produced!$',
                     stdout, re.MULTILINE):
            print(stdout, file=sys.stderr)
            raise TaskError('failed to extract output name from latex log')

        # LuaTeX (0.76.0) doesn't include the output directory in the
        # logged transcript or output file name.
        if os.path.basename(jobname) == jobname and \
           os.path.exists(os.path.join(self.__obj_dir, jobname + '.log')):
            jobname = os.path.join(self.__obj_dir, jobname)
            if outname is not None:
                outname = os.path.join(self.__obj_dir, outname)

        return jobname, outname

    def __parse_recorder(self, jobname):
        """Parse file recorder output."""
        # XXX If latex fails because a file isn't found, that doesn't
        # go into the .fls file, but creating that file will affect
        # the computation, so it should be included as an input.
        # Though it's generally true that files can be added earlier
        # in search paths and will affect the output without us knowing.
        #
        # XXX This is a serious problem for bibtex, since the first
        # run won't depend on the .bbl file!  But maybe the .aux file
        # will always cause a re-run, at which point the .bbl will
        # exist?
        filename = jobname + '.fls'
        try:
            recorder = open(filename)
        except OSError as e:
            raise TaskError('failed to open file recorder output: ' + str(e)) \
                from e
        pwd, inputs, outputs = '', set(), set()
        for linenum, line in enumerate(recorder):
            parts = line.rstrip('\n').split(' ', 1)
            if parts[0] == 'PWD':
                pwd = parts[1]
            elif parts[0] in ('INPUT', 'OUTPUT'):
                if parts[1].startswith('/'):
                    path = parts[1]
                else:
                    # Try to make "nice" paths, especially for clean
                    path = os.path.relpath(os.path.join(pwd, parts[1]))
                if parts[0] == 'INPUT':
                    inputs.add(path)
                else:
                    outputs.add(path)
            else:
                raise TaskError('syntax error on line {} of {}'
                                .format(linenum, filename))
        # Ironically, latex omits the .fls file itself
        outputs.add(filename)
        outputs.add(jobname + '.synctex.gz') # synctex is not recorded
        return inputs, outputs

    def __create_outdirs(self, stdout):
        # In some cases, such as \include'ing a file from a
        # subdirectory, TeX will attempt to create files in
        # subdirectories of the output directory that don't exist.
        # Detect this, create the output directory, and re-run.
        m = re.search('^! I can\'t write on file `(.*)\'\\.$', stdout, re.M)
        if m and m.group(1).find('/') > 0 and '../' not in m.group(1):
            debug('considering creating output sub-directory for {}'.
                  format(m.group(1)))
            subdir = os.path.dirname(m.group(1))
            newdir = os.path.join(self.__obj_dir, subdir)
            if os.path.isdir(subdir) and not os.path.isdir(newdir):
                debug('creating output subdirectory {}'.format(newdir))
                try:
                    mkdir_p(newdir)
                except OSError as e:
                    raise TaskError('failed to create output subdirectory: ' +
                                    str(e)) from e
                self._input('unstable')
                return True

    def report(self):
        extra = self._get_result_extra()
        if extra is None:
            return 0

        # Parse the log
        logfile = open(extra['jobname'] + '.log', 'rt', errors='surrogateescape')
        for msg in self.__clean_messages(
                LaTeXFilter(self.__nowarns).feed(
                    logfile.read(), True).get_messages()):
            msg.emit()

        # Return LaTeX's exit status
        return extra['status']

    def __clean_messages(self, msgs):
        """Make some standard log messages more user-friendly."""
        have_undefined_reference = False
        for msg in msgs:
            if msg.msg == '==> Fatal error occurred, no output PDF file produced!':
                msg = msg._replace(typ='info',
                                   msg='Fatal error (no output file produced)')
            if msg.msg.startswith('[LaTeX] '):
                # Strip unnecessary package name
                msg = msg._replace(msg=msg.msg.split(' ', 1)[1])
            if re.match(r'Reference .* undefined', msg.msg):
                have_undefined_reference = True
            if have_undefined_reference and \
               re.match(r'There were undefined references', msg.msg):
                # LaTeX prints this at the end so the user knows it's
                # worthwhile looking back at the log.  Since latexrun
                # makes the earlier messages obvious, this is
                # redundant.
                continue
            yield msg

    def get_tex_filename(self):
        return self.__tex_filename

    def get_jobname(self):
        extra = self._get_result_extra()
        if extra is None:
            return None
        return extra['jobname']

    def get_outname(self):
        extra = self._get_result_extra()
        if extra is None:
            return None
        return extra['outname']

    def get_status(self):
        extra = self._get_result_extra()
        if extra is None:
            return None
        return extra['status']

class LaTeXCommit(Task):
    def __init__(self, db, latex_task, output_path):
        super().__init__(db, 'latex_commit::' +
                         normalize_input_path(latex_task.get_tex_filename()))
        self.__latex_task = latex_task
        self.__output_path = output_path
        self.status = 'There were errors'

    def _input_latex(self):
        return self.__latex_task.get_status(), self.__latex_task.get_outname()

    def _execute(self):
        self.status = 'There were errors'

        # If latex succeeded with output, atomically commit the output
        status, outname = self._input('latex')
        if status != 0 or outname is None:
            debug('not committing (status {}, outname {})', status, outname)
            if outname is None:
                self.status = 'No pages of output'
            return RunResult([], None)

        commit = self.__output_path or os.path.basename(outname)
        if os.path.abspath(commit) == os.path.abspath(outname):
            debug('skipping commit (outname is commit name)')
            self.status = None
            return RunResult([], None)

        try:
            if os.path.exists(commit) and filecmp.cmp(outname, commit):
                debug('skipping commit ({} and {} are identical)',
                      outname, commit)
                # To avoid confusion, touch the output file
                open(outname, 'r+b').close()
            else:
                debug('commiting {} to {}', outname, commit)
                shutil.copy(outname, outname + '~')
                os.rename(outname + '~', commit)
        except OSError as e:
            raise TaskError('error committing latex output: {}'.format(e)) from e
        self._input('file', outname)
        self.status = None
        return RunResult([commit], None)

class LaTeXFilter:
    TRACE = False               # Set to enable detailed parse tracing

    def __init__(self, nowarns=[]):
        self.__data = ''
        self.__restart_pos = 0
        self.__restart_file_stack = []
        self.__restart_messages_len = 0
        self.__messages = []
        self.__first_file = None
        self.__fatal_error = False
        self.__missing_includes = False
        self.__pageno = 1
        self.__restart_pageno = 1

        self.__suppress = {cls: 0 for cls in nowarns}

    def feed(self, data, eof=False):
        """Feed LaTeX log data to the parser.

        The log data can be from LaTeX's standard output, or from the
        log file.  If there will be no more data, set eof to True.
        """

        self.__data += data
        self.__data_complete = eof

        # Reset to last known-good restart point
        self.__pos = self.__restart_pos
        self.__file_stack = self.__restart_file_stack.copy()
        self.__messages = self.__messages[:self.__restart_messages_len]
        self.__lstart = self.__lend = -1
        self.__pageno = self.__restart_pageno

        # Parse forward
        while self.__pos < len(self.__data):
            self.__noise()

        # Handle suppressed warnings
        if eof:
            msgs = ['%d %s warning%s' % (count, cls, "s" if count > 1 else "")
                    for cls, count in self.__suppress.items() if count]
            if msgs:
                self.__message('info', None,
                               '%s not shown (use -Wall to show them)' %
                               ', '.join(msgs), filename=self.__first_file)

        if eof and len(self.__file_stack) and not self.__fatal_error:
            # Fatal errors generally cause TeX to "succumb" without
            # closing the file stack, so don't complain in that case.
            self.__message('warning', None,
                           "unbalanced `(' in log; file names may be wrong")
        return self

    def get_messages(self):
        """Return a list of warning and error Messages."""
        return self.__messages

    def get_file_stack(self):
        """Return the file stack for the data that has been parsed.

        This results a list from outermost file to innermost file.
        The list may be empty.
        """

        return self.__file_stack

    def has_missing_includes(self):
        """Return True if the log reported missing \\include files."""
        return self.__missing_includes

    def __save_restart_point(self):
        """Save the current state as a known-good restart point.

        On the next call to feed, the parser will reset to this point.
        """
        self.__restart_pos = self.__pos
        self.__restart_file_stack = self.__file_stack.copy()
        self.__restart_messages_len = len(self.__messages)
        self.__restart_pageno = self.__pageno

    def __message(self, typ, lineno, msg, cls=None, filename=None):
        if cls is not None and cls in self.__suppress:
            self.__suppress[cls] += 1
            return
        filename = filename or (self.__file_stack[-1] if self.__file_stack
                                else self.__first_file)
        self.__messages.append(Message(typ, filename, lineno, msg))

    def __ensure_line(self):
        """Update lstart and lend."""
        if self.__lstart <= self.__pos < self.__lend:
            return
        self.__lstart = self.__data.rfind('\n', 0, self.__pos) + 1
        self.__lend = self.__data.find('\n', self.__pos) + 1
        if self.__lend == 0:
            self.__lend = len(self.__data)

    @property
    def __col(self):
        """The 0-based column number of __pos."""
        self.__ensure_line()
        return self.__pos - self.__lstart

    @property
    def __avail(self):
        return self.__pos < len(self.__data)

    def __lookingat(self, needle):
        return self.__data.startswith(needle, self.__pos)

    def __lookingatre(self, regexp, flags=0):
        return re.compile(regexp, flags=flags).match(self.__data, self.__pos)

    def __skip_line(self):
        self.__ensure_line()
        self.__pos = self.__lend

    def __consume_line(self, unwrap=False):
        self.__ensure_line()
        data = self.__data[self.__pos:self.__lend]
        self.__pos = self.__lend
        if unwrap:
            # TeX helpfully wraps all terminal output at 79 columns
            # (max_print_line).  If requested, unwrap it.  There's
            # simply no way to do this perfectly, since there could be
            # a line that happens to be 79 columns.
            #
            # We check for >=80 because a bug in LuaTeX causes it to
            # wrap at 80 columns instead of 79 (LuaTeX #900).
            while self.__lend - self.__lstart >= 80:
                if self.TRACE: print('<{}> wrapping'.format(self.__pos))
                self.__ensure_line()
                data = data[:-1] + self.__data[self.__pos:self.__lend]
                self.__pos = self.__lend
        return data

    # Parser productions

    def __noise(self):
        # Most of TeX's output is line noise that combines error
        # messages, warnings, file names, user errors and warnings,
        # and echos of token lists and other input.  This attempts to
        # tease these apart, paying particular attention to all of the
        # places where TeX echos input so that parens in the input do
        # not confuse the file name scanner.  There are three
        # functions in TeX that echo input: show_token_list (used by
        # runaway and show_context, which is used by print_err),
        # short_display (used by overfull/etc h/vbox), and show_print
        # (used in issue_message and the same places as
        # show_token_list).
        lookingat, lookingatre = self.__lookingat, self.__lookingatre
        if self.__col == 0:
            # The following messages are always preceded by a newline
            if lookingat('! '):
                return self.__errmessage()
            if lookingat('!pdfTeX error: '):
                return self.__pdftex_fail()
            if lookingat('Runaway '):
                return self.__runaway()
            if lookingatre(r'(Overfull|Underfull|Loose|Tight) \\[hv]box \('):
                return self.__bad_box()
            if lookingatre('(Package |Class |LaTeX |pdfTeX )?(\w+ )?warning: ', re.I):
                return self.__generic_warning()
            if lookingatre('No file .*\\.tex\\.$', re.M):
                # This happens with \includes of missing files.  For
                # whatever reason, LaTeX doesn't consider this even
                # worth a warning, but I do!
                self.__message('warning', None,
                               self.__simplify_message(
                                   self.__consume_line(unwrap=True).strip()))
                self.__missing_includes = True
                return
            # Other things that are common and irrelevant
            if lookingatre(r'(Package|Class|LaTeX) (\w+ )?info: ', re.I):
                return self.__generic_info()
            if lookingatre(r'(Document Class|File|Package): '):
                # Output from "\ProvidesX"
                return self.__consume_line(unwrap=True)
            if lookingatre(r'\\\w+=\\[a-z]+\d+\n'):
                # Output from "\new{count,dimen,skip,...}"
                return self.__consume_line(unwrap=True)

        # print(self.__data[self.__lstart:self.__lend].rstrip())
        # self.__pos = self.__lend
        # return

        # Now that we've substantially reduced the spew and hopefully
        # eliminated all input echoing, we're left with the file name
        # stack, page outs, and random other messages from both TeX
        # and various packages.  We'll assume at this point that all
        # parentheses belong to the file name stack or, if they're in
        # random other messages, they're at least balanced and nothing
        # interesting happens between them.  For page outs, ship_out
        # prints a space if not at the beginning of a line, then a
        # "[", then the page number being shipped out (this is
        # usually, but not always, followed by "]").
        m = re.compile(r'[(){}\n]|(?<=[\n ])\[\d+', re.M).\
            search(self.__data, self.__pos)
        if m is None:
            self.__pos = len(self.__data)
            return
        self.__pos = m.start() + 1
        ch = self.__data[m.start()]
        if ch == '\n':
            # Save this as a known-good restart point for incremental
            # parsing, since we definitely didn't match any of the
            # known message types above.
            self.__save_restart_point()
        elif ch == '[':
            # This is printed at the end of a page, so we're beginning
            # page n+1.
            self.__pageno = int(self.__lookingatre(r'\d+').group(0)) + 1
        elif ((self.__data.startswith('`', m.start() - 1) or
               self.__data.startswith('`\\', m.start() - 2)) and
               self.__data.startswith('\'', m.start() + 1)):
            # (, ), {, and } sometimes appear in TeX's error
            # descriptions, but they're always in `'s (and sometimes
            # backslashed)
            return
        elif ch == '(':
            # XXX Check that the stack doesn't drop to empty and then re-grow
            first = self.__first_file is None and self.__col == 1
            filename = self.__filename()
            self.__file_stack.append(filename)
            if first:
                self.__first_file = filename
            if self.TRACE:
                print('<{}>{}enter {}'.format(
                    m.start(), ' '*len(self.__file_stack), filename))
        elif ch == ')':
            if len(self.__file_stack):
                if self.TRACE:
                    print('<{}>{}exit {}'.format(
                        m.start(), ' '*len(self.__file_stack),
                        self.__file_stack[-1]))
                self.__file_stack.pop()
            else:
                self.__message('warning', None,
                               "extra `)' in log; file names may be wrong")
        elif ch == '{':
            # TeX uses this for various things we want to ignore, like
            # file names and print_mark.  Consume up to the '}'
            lax_checking = "strict-parse" in self.__suppress
            epos = nested_parenthesis_end(self.__data[self.__pos-1:], '{[(', '}])',
                                          lax_checking=lax_checking)
            if epos == -1:
                self.__message('warning', None,
                               "unbalanced `{' in log; file names may be wrong")
            self.__pos += epos + 1
        elif ch == '}':
            self.__message('warning', None,
                           "extra `}' in log; file names may be wrong")

    def __filename(self):
        initcol = self.__col
        first = True
        name = ''
        # File names may wrap, but if they do, TeX will always print a
        # newline before the open paren
        while first or (initcol == 1 and self.__lookingat('\n')
                        and self.__col >= 79):
            if not first:
                self.__pos += 1
            m = self.__lookingatre(r'[^(){} \n]*')
            name += m.group()
            self.__pos = m.end()
            first = False
        return name

    def __simplify_message(self, msg):
        msg = re.sub(r'^(?:Package |Class |LaTeX |pdfTeX )?([^ ]+) (?:Error|Warning): ',
                     r'[\1] ', msg, flags=re.I)
        msg = re.sub(r'\.$', '', msg)
        msg = re.sub(r'has occurred (while \\output is active)', r'\1', msg)
        return msg

    def __errmessage(self):
        # Procedure print_err (including \errmessage, itself used by
        # LaTeX's \GenericError and all of its callers), as well as
        # fatal_error.  Prints "\n!  " followed by error text
        # ("Emergency stop" in the case of fatal_error).  print_err is
        # always followed by a call to error, which prints a period,
        # and a newline...
        msg = self.__consume_line(unwrap=True)[1:].strip()
        is_fatal_error = (msg == 'Emergency stop.')
        msg = self.__simplify_message(msg)
        # ... and then calls show_context, which prints the input
        # stack as pairs of lines giving the context.  These context
        # lines are truncated so they never wrap.  Each pair of lines
        # will start with either "<something> " if the context is a
        # token list, "<*> " for terminal input (or command line),
        # "<read ...>" for stream reads, something like "\macroname
        # #1->" for macros (though everything after \macroname is
        # subject to being elided as "..."), or "l.[0-9]+ " if it's a
        # file.  This is followed by the errant input with a line
        # break where the error occurred.
        lineno = None
        found_context = False
        stack = []
        while self.__avail:
            m1 = self.__lookingatre(r'<([a-z ]+|\*|read [^ >]*)> |\\.*(->|...)')
            m2 = self.__lookingatre('l\.[0-9]+ ')
            if m1:
                found_context = True
                pre = self.__consume_line().rstrip('\n')
                stack.append(pre)
            elif m2:
                found_context = True
                pre = self.__consume_line().rstrip('\n')
                info, rest = pre.split(' ', 1)
                lineno = int(info[2:])
                stack.append(rest)
            elif found_context:
                # Done with context
                break
            if found_context:
                # Consume the second context line
                post = self.__consume_line().rstrip('\n')
                # Clean up goofy trailing ^^M TeX sometimes includes
                post = re.sub(r'\^\^M$', '', post)
                if post[:len(pre)].isspace() and not post.isspace():
                    stack.append(len(stack[-1]))
                    stack[-2] += post[len(pre):]
            else:
                # If we haven't found the context, skip the line.
                self.__skip_line()
        stack_msg = ''
        for i, trace in enumerate(stack):
            stack_msg += ('\n         ' + (' ' * trace) + '^'
                          if isinstance(trace, int) else
                          '\n      at ' + trace.rstrip() if i == 0 else
                          '\n    from ' + trace.rstrip())

        if is_fatal_error:
            # fatal_error always prints one additional line of message
            info = self.__consume_line().strip()
            if info.startswith('*** '):
                info = info[4:]
            msg += ': '  + info.lstrip('(').rstrip(')')

        self.__message('error', lineno, msg + stack_msg)
        self.__fatal_error = True

    def __pdftex_fail(self):
        # Procedure pdftex_fail.  Prints "\n!pdfTeX error: ", the
        # message, and a newline.  Unlike print_err, there's never
        # context.
        msg = self.__consume_line(unwrap=True)[1:].strip()
        msg = self.__simplify_message(msg)
        self.__message('error', None, msg)

    def __runaway(self):
        # Procedure runaway.  Prints "\nRunaway ...\n" possibly
        # followed by token list (user text).  Always followed by a
        # call to print_err, so skip lines until we see the print_err.
        self.__skip_line()      # Skip "Runaway ...\n"
        if not self.__lookingat('! ') and self.__avail:
            # Skip token list, which is limited to one line
            self.__skip_line()

    def __bad_box(self):
        # Function hpack and vpack.  hpack prints a warning, a
        # newline, then a short_display of the offending text.
        # Unfortunately, there's nothing indicating the end of the
        # offending text, but it should be on one (possible wrapped)
        # line.  vpack prints a warning and then, *unless output is
        # active*, a newline.  The missing newline is probably a bug,
        # but it sure makes our lives harder.
        origpos = self.__pos
        msg = self.__consume_line()
        m = re.search(r' in (?:paragraph|alignment) at lines ([0-9]+)--([0-9]+)', msg) or \
            re.search(r' detected at line ([0-9]+)', msg)
        if m:
            # Sometimes TeX prints crazy line ranges like "at lines
            # 8500--250".  The lower number seems roughly sane, so use
            # that.  I'm not sure what causes this, but it may be
            # related to shipout routines messing up line registers.
            lineno = min(int(m.group(1)), int(m.groups()[-1]))
            msg = msg[:m.start()]
        else:
            m = re.search(r' while \\output is active', msg)
            if m:
                lineno = None
                msg = msg[:m.end()]
            else:
                self.__message('warning', None,
                               'malformed bad box message in log')
                return
        # Back up to the end of the known message text
        self.__pos = origpos + m.end()
        if self.__lookingatre(r'\s*\n'):
            # We have a newline, so consume it and look for the
            # offending text.
            self.__pos += 1
            # If there is offending text, it will start with a font
            # name, which will start with a \.
            if 'hbox' in msg and self.__lookingatre(r'(\[\]\s?)*\s*\\'):
                consumed = self.__consume_line(unwrap=True)
                if self.TRACE: print('consuming `<{}>\''.format(consumed))
        msg = self.__simplify_message(msg) + ' (page {})'.format(self.__pageno)
        cls = msg.split(None, 1)[0].lower()
        self.__message('warning', lineno, msg, cls=cls)

    def __generic_warning(self):
        # Warnings produced by LaTeX's \GenericWarning (which is
        # called by \{Package,Class}Warning and \@latex@warning),
        # warnings produced by pdftex_warn, and other random warnings.
        msg, cls = self.__generic_info()
        # Most warnings include an input line emitted by \on@line
        m = re.search(' on input line ([0-9]+)', msg)
        if m:
            lineno = int(m.group(1))
            msg = msg[:m.start()]
        else:
            lineno = None
        msg = self.__simplify_message(msg)
        self.__message('warning', lineno, msg, cls=cls)

    def __generic_info(self):
        # Messages produced by LaTeX's \Generic{Error,Warning,Info}
        # and things that look like them
        msg = self.__consume_line(unwrap=True).strip()
        # Package and class messages are continued with lines
        # containing '(package name)            '
        pkg_name = msg.split(' ', 2)[1]
        prefix = '(' + pkg_name + ')            '
        while self.__lookingat(prefix):
            # Collect extra lines.  It's important that we keep these
            # because they may contain context information like line
            # numbers.
            extra = self.__consume_line(unwrap=True)
            msg += ' ' + extra[len(prefix):].strip()
        return msg, pkg_name.lower()

##################################################################
# BibTeX task
#

class BibTeX(Task):
    def __init__(self, db, latex_task, cmd, cmd_args, nowarns, obj_dir):
        super().__init__(db, 'bibtex::' + normalize_input_path(
            latex_task.get_tex_filename()))
        self.__latex_task = latex_task
        self.__cmd = cmd
        self.__cmd_args = cmd_args
        self.__obj_dir = obj_dir

    def stable(self):
        # If bibtex doesn't have its inputs, then it's stable because
        # it has no effect on system state.
        jobname = self.__latex_task.get_jobname()
        if jobname is None:
            # We don't know where the .aux file is until latex has run
            return True
        if not os.path.exists(jobname + '.aux'):
            # Input isn't ready, so bibtex will simply fail without
            # affecting system state.  Hence, this task is trivially
            # stable.
            return True
        if not self.__find_bib_cmds(os.path.dirname(jobname), jobname + '.aux'):
            # The tex file doesn't refer to any bibliographic data, so
            # don't run bibtex.
            return True

        return super().stable()

    def __find_bib_cmds(self, basedir, auxname, stack=()):
        debug('scanning for bib commands in {}'.format(auxname))
        if auxname in stack:
            raise TaskError('.aux file loop')
        stack = stack + (auxname,)

        try:
            aux_data = open(auxname, errors='surrogateescape').read()
        except FileNotFoundError:
            # The aux file may not exist if latex aborted
            return False
        if re.search(r'^\\bibstyle\{', aux_data, flags=re.M) or \
           re.search(r'^\\bibdata\{',  aux_data, flags=re.M):
            return True

        if re.search(r'^\\abx@aux@cite\{', aux_data, flags=re.M):
            # biber citation
            return True

        # Recurse into included aux files (see aux_input_command), in
        # case \bibliography appears in an \included file.
        for m in re.finditer(r'^\\@input\{([^}]*)\}', aux_data, flags=re.M):
            if self.__find_bib_cmds(basedir, os.path.join(basedir, m.group(1)),
                                    stack):
                return True

        return False

    def _input_args(self):
        if self.__is_biber():
            aux_name = os.path.basename(self.__latex_task.get_jobname())
        else:
            aux_name = os.path.basename(self.__latex_task.get_jobname()) + '.aux'
        return [self.__cmd] + self.__cmd_args + [aux_name]

    def _input_cwd(self):
        return os.path.dirname(self.__latex_task.get_jobname())

    def _input_auxfile(self, auxname):
        # We don't consider the .aux files regular inputs.
        # Instead, we extract just the bit that BibTeX cares about
        # and depend on that.  See get_aux_command_and_process in
        # bibtex.web.
        debug('hashing filtered aux file {}', auxname)
        try:
            with open(auxname, 'rb') as aux:
                h = hashlib.sha256()
                for line in aux:
                    if line.startswith((b'\\citation{', b'\\bibdata{',
                                        b'\\bibstyle{', b'\\@input{',
                                        b'\\abx@aux@cite{')):
                        h.update(line)
                return h.hexdigest()
        except FileNotFoundError:
            debug('{} does not exist', auxname)
            return None

    def __path_join(self, first, rest):
        if rest is None:
            # Append ':' to keep the default search path
            return first + ':'
        return first + ':' + rest

    def __is_biber(self):
        return "biber" in self.__cmd

    def _execute(self):
        # This gets complicated when \include is involved.  \include
        # switches to a different aux file and records its path in the
        # main aux file.  However, BibTeX does not consider this path
        # to be relative to the location of the main aux file, so we
        # have to run BibTeX *in the output directory* for it to
        # follow these includes (there's no way to tell BibTeX other
        # locations to search).  Unfortunately, this means BibTeX will
        # no longer be able to find local bib or bst files, but so we
        # tell it where to look by setting BIBINPUTS and BSTINPUTS
        # (luckily we can control this search).  We have to pass this
        # same environment down to Kpathsea when we resolve the paths
        # in BibTeX's log.
        args, cwd = self._input('args'), self._input('cwd')
        debug('running {} in {}', args, cwd)

        env = os.environ.copy()
        env['BIBINPUTS'] = self.__path_join(os.getcwd(), env.get('BIBINPUTS'))
        env['BSTINPUTS'] = self.__path_join(os.getcwd(), env.get('BSTINPUTS'))

        try:
            verbose_cmd(args, cwd, env)
            p = subprocess.Popen(args, cwd=cwd, env=env,
                                 stdin=subprocess.DEVNULL,
                                 stdout=subprocess.PIPE,
                                 stderr=subprocess.STDOUT)
            stdout = self.__feed_terminal(p.stdout)
            status = p.wait()
        except OSError as e:
            raise TaskError('failed to execute bibtex task: ' + str(e)) from e

        inputs, auxnames, outbase = self.__parse_inputs(stdout, cwd, env)
        if not inputs and not auxnames:
            # BibTeX failed catastrophically.
            print(stdout, file=sys.stderr)
            raise TaskError('failed to execute bibtex task')

        # Register environment variable inputs
        for env_var in ['TEXMFOUTPUT', 'BSTINPUTS', 'BIBINPUTS', 'PATH']:
            self._input('env', env_var)

        # Register file inputs
        for path in auxnames:
            self._input('auxfile', path)
        for path in inputs:
            self._input('file', path)

        if self.__is_biber():
            outbase = os.path.join(cwd, outbase)
        outputs = [outbase + '.bbl', outbase + '.blg']
        return RunResult(outputs, {'outbase': outbase, 'status': status,
                                   'inputs': inputs})

    def __feed_terminal(self, stdout):
        with Progress('bibtex') as progress:
            buf, linebuf = [], ''
            while True:
                data = os.read(stdout.fileno(), 4096)
                if not data:
                    break
                # See "A note about encoding" above
                data = data.decode('ascii', errors='surrogateescape')
                buf.append(data)
                linebuf += data
                while '\n' in linebuf:
                    line, _, linebuf = linebuf.partition('\n')
                    if line.startswith('Database file'):
                        progress.update(line.split(': ', 1)[1])
        return ''.join(buf)

    def __parse_inputs(self, log, cwd, env):
        # BibTeX conveniently logs every file that it opens, and its
        # log is actually sensible (see calls to a_open_in in
        # bibtex.web.)  The only trick is that these file names are
        # pre-kpathsea lookup and may be relative to the directory we
        # ran BibTeX in.
        #
        # Because BibTeX actually depends on very little in the .aux
        # file (and it's likely other things will change in the .aux
        # file), we don't count the whole .aux file as an input, but
        # instead depend only on the lines that matter to BibTeX.
        kpathsea = Kpathsea('bibtex')
        inputs = []
        auxnames = []
        outbase = None
        for line in log.splitlines():
            m = re.match('(?:The top-level auxiliary file:'
                         '|A level-[0-9]+ auxiliary file:) (.*)', line)
            if m:
                auxnames.append(os.path.join(cwd, m.group(1)))
                continue
            m = re.match('(?:(The style file:)|(Database file #[0-9]+:)) (.*)',
                         line)
            if m:
                filename = m.group(3)
                if m.group(1):
                    filename = kpathsea.find_file(filename, 'bst', cwd, env)
                elif m.group(2):
                    filename = kpathsea.find_file(filename, 'bib', cwd, env)

                # If this path is relative to the source directory,
                # clean it up for error reporting and portability of
                # the dependency DB
                if filename.startswith('/'):
                    relname = os.path.relpath(filename)
                    if '../' not in relname:
                        filename = relname

                inputs.append(filename)

            # biber output
            m = re.search("Found BibTeX data source '(.*?)'",
                         line)
            if m:
                filename = m.group(1)
                inputs.append(filename)

            m = re.search("Logfile is '(.*?)'", line)
            if m:
                outbase = m.group(1)[:-4]

        if outbase is None:
            outbase = auxnames[0][:-4]

        return inputs, auxnames, outbase

    def report(self):
        extra = self._get_result_extra()
        if extra is None:
            return 0

        # Parse and pretty-print the log
        log = open(extra['outbase'] + '.blg', 'rt').read()
        inputs = extra['inputs']
        for msg in BibTeXFilter(log, inputs).get_messages():
            msg.emit()

        # BibTeX exits with 1 if there are warnings, 2 if there are
        # errors, and 3 if there are fatal errors (sysdep.h).
        # Translate to a normal UNIX exit status.
        if extra['status'] >= 2:
            return 1
        return 0

class BibTeXFilter:
    def __init__(self, data, inputs):
        self.__inputs = inputs
        self.__key_locs = None

        self.__messages = []

        prev_line = ''
        for line in data.splitlines():
            msg = self.__process_line(prev_line, line)
            if msg is not None:
                self.__messages.append(Message(*msg))
            prev_line = line

    def get_messages(self):
        """Return a list of warning and error Messages."""
        # BibTeX reports most errors in no particular order.  Sort by
        # file and line.
        return sorted(self.__messages,
                      key=lambda msg: (msg.filename or '', msg.lineno or 0))

    def __process_line(self, prev_line, line):
        m = None
        def match(regexp):
            nonlocal m
            m = re.match(regexp, line)
            return m

        # BibTeX has many error paths, but luckily the set is closed,
        # so we can find all of them.  This first case is the
        # workhorse format.
        #
        # AUX errors: aux_err/aux_err_return/aux_err_print
        #
        # BST errors: bst_ln_num_print/bst_err/
        # bst_err_print_and_look_for_blank_line_return/
        # bst_warn_print/bst_warn/
        # skip_token/skip_token_print/
        # bst_ext_warn/bst_ext_warn_print/
        # bst_ex_warn/bst_ex_warn_print/
        # bst_mild_ex_warn/bst_mild_ex_warn_print/
        # bst_string_size_exceeded
        #
        # BIB errors: bib_ln_num_print/
        # bib_err_print/bib_err/
        # bib_warn_print/bib_warn/
        # bib_one_of_two_expected_err/macro_name_warning/
        if match('(.*?)---?line ([0-9]+) of file (.*)'):
            # Sometimes the real error is printed on the previous line
            if m.group(1) == 'while executing':
                # bst_ex_warn.  The real message is on the previous line
                text = prev_line
            else:
                text = m.group(1) or prev_line
            typ, msg = self.__canonicalize(text)
            return (typ, m.group(3), int(m.group(2)), msg)

        # overflow/print_overflow
        if match('Sorry---you\'ve exceeded BibTeX\'s (.*)'):
            return ('error', None, None, 'capacity exceeded: ' + m.group(1))
        # confusion/print_confusion
        if match('(.*)---this can\'t happen$'):
            return ('error', None, None, 'internal error: ' + m.group(1))
        # aux_end_err
        if match('I found (no .*)---while reading file (.*)'):
            return ('error', m.group(2), None, m.group(1))
        # bad_cross_reference_print/
        # nonexistent_cross_reference_error/
        # @<Complain about a nested cross reference@>
        #
        # This is split across two lines.  Match the second.
        if match('^refers to entry "'):
            typ, msg = self.__canonicalize(prev_line + ' ' + line)
            msg = re.sub('^a (bad cross reference)', '\\1', msg)
            # Try to give this key a location
            filename = lineno = None
            m2 = re.search(r'--entry "[^"]"', prev_line)
            if m2:
                filename, lineno = self.__find_key(m2.group(1))
            return (typ, filename, lineno, msg)
        # print_missing_entry
        if match('Warning--I didn\'t find a database entry for (".*")'):
            return ('warning', None, None,
                    'no database entry for ' + m.group(1))
        # x_warning
        if match('Warning--(.*)'):
            # Most formats give warnings about "something in <key>".
            # Try to match it up.
            filename = lineno = None
            for m2 in reversed(list(re.finditer(r' in ([^, \t\n]+)\b', line))):
                if m2:
                    filename, lineno = self.__find_key(m2.group(1))
                    if filename:
                        break
            return ('warning', filename, lineno, m.group(1))
        # @<Clean up and leave@>
        if match('Aborted at line ([0-9]+) of file (.*)'):
            return ('info', m.group(2), int(m.group(1)), 'aborted')

        # biber type errors
        if match('^.*> WARN - (.*)$'):
            print ('warning', None, None, m.group(1))
            m2 = re.match("(.*) in file '(.*?)', skipping ...", m.group(1))
            if m2:
                return ('warning', m2.group(2), "0", m2.group(1))
            return ('warning', None, None, m.group(1))

        if match('^.*> ERROR - (.*)$'):
            m2 = re.match("BibTeX subsystem: (.*?), line (\d+), (.*)$", m.group(1))
            if m2:
                return ('error', m2.group(1), m2.group(2), m2.group(3))
            return ('error', None, None, m.group(1))


    def __canonicalize(self, msg):
        if msg.startswith('Warning'):
            msg = re.sub('^Warning-*', '', msg)
            typ = 'warning'
        else:
            typ = 'error'
        msg = re.sub('^I(\'m| was)? ', '', msg)
        msg = msg[:1].lower() + msg[1:]
        return typ, msg

    def __find_key(self, key):
        if self.__key_locs is None:
            p = BibTeXKeyParser()
            self.__key_locs = {}
            for filename in self.__inputs:
                data = open(filename, 'rt', errors='surrogateescape').read()
                for pkey, lineno in p.parse(data):
                    self.__key_locs.setdefault(pkey, (filename, lineno))
        return self.__key_locs.get(key, (None, None))

class BibTeXKeyParser:
    """Just enough of a BibTeX parser to find keys."""

    def parse(self, data):
        IDENT_RE = '(?![0-9])([^\x00-\x20\x80-\xff \t"#%\'(),={}]+)'
        self.__pos, self.__data = 0, data
        # Find the next entry
        while self.__consume('[^@]*@[ \t\n]*'):
            # What type of entry?
            if not self.__consume(IDENT_RE + '[ \t\n]*'):
                continue
            typ = self.__m.group(1)
            if typ == 'comment':
                continue
            start = self.__pos
            if not self.__consume('([{(])[ \t\n]*'):
                continue
            closing, key_re = {'{' : ('}', '([^, \t\n}]*)'),
                               '(' : (')', '([^, \t\n]*)')}[self.__m.group(1)]
            if typ not in ('preamble', 'string'):
                # Regular entry; get key
                if self.__consume(key_re):
                    yield self.__m.group(1), self.__lineno()
            # Consume body of entry
            self.__pos = start
            self.__balanced(closing)

    def __consume(self, regexp):
        self.__m = re.compile(regexp).match(self.__data, self.__pos)
        if self.__m:
            self.__pos = self.__m.end()
        return self.__m

    def __lineno(self):
        return self.__data.count('\n', 0, self.__pos) + 1

    def __balanced(self, closing):
        self.__pos += 1
        level = 0
        skip = re.compile('[{}' + closing + ']')
        while True:
            m = skip.search(self.__data, self.__pos)
            if not m:
                break
            self.__pos = m.end()
            ch = m.group(0)
            if level == 0 and ch == closing:
                break
            elif ch == '{':
                level += 1
            elif ch == '}':
                level -= 1

class Kpathsea:
    def __init__(self, program_name):
        self.__progname = program_name

    def find_file(self, name, format, cwd=None, env=None):
        """Return the resolved path of 'name' or None."""

        args = ['kpsewhich', '-progname', self.__progname, '-format', format,
                name]
        try:
            verbose_cmd(args, cwd, env)
            path = subprocess.check_output(
                args, cwd=cwd, env=env, universal_newlines=True).strip()
        except subprocess.CalledProcessError as e:
            if e.returncode != 1:
                raise
            return None
        if cwd is None:
            return path
        return os.path.join(cwd, path)

if __name__ == "__main__":
    main()


==> bin/mkabstract <==
#!/usr/bin/env python3

import os
import sys
import re
import textwrap

if len(sys.argv) != 3:
    print("[usage] %s [p.tex] [abstract.tex]" % sys.argv[0])
    exit(0)

pn_main = sys.argv[1]
pn_abst = sys.argv[2]

def get_keywords(tex):
    rtn = {}
    tok = re.findall(r"\\newcommand{\\([^}]+)}{(.*)}", tex)
    for (k, v) in tok:
        # clean up v
        v = v.replace("\\mbox{", "")
        v = v.replace("\\textsc{", "")
        v = v.replace("\\cc{", "")
        v = v.replace("\\xspace", "")
        v = v.replace("}", "")
        v = v.replace("{", "")
        v = v.replace("\\", "")
        rtn[k] = v
    return rtn

def get_sys(tex):
    tok = re.findall(r"\\newcommand{\\sys}{\\mbox{\\textsc{([^}]*)}", tex)
    if len(tok) == 0:
        print("Failed to find 'sys'")
        exit(1)
    return tok[0]

kw = get_keywords(open(pn_main).read())

abstract = []
for l in open(pn_abst):
    l = l.strip()
    if l.startswith("%"):
        continue
    if l.endswith("%"):
        l = l[:-1]

    if "{abstract}" in l:
        continue
    l = l.replace("\\%", "%")
    l = l.replace("\\emph{", "")
    l = l.replace("\\cc{", "")
    l = l.replace("{", "")
    l = l.replace("}", "")
    l = l.replace("~", " ")
    l = l.replace("\\,", " ")
    l = l.replace("\\X", "x")
    l = l.replace("\\&", "&")
    l = l.replace("\\@", "")
    l = l.replace("\\$", "$")
    l = l.replace("---", " -- ")
    l = l.replace("--", "-")
    l = l.replace("``", "'")
    l = l.replace("''", "'")
    l = l.replace("\\ie", "i.e.")
    l = l.replace("\\eg", "e.g.")
    l = l.replace("\\etal", " et al.")
    l = l.replace("\\Bs", " B/s")
    l = l.replace("\\KBs", " KB/s")
    l = l.replace("\\MBs", " MB/s")
    l = l.replace("\\GBs", " GB/s")
    l = l.replace("\\KB", " KB")
    l = l.replace("\\MB", " MB")
    l = l.replace("\\GB", " GB")
    l = l.replace("\\TB", " TB")
    l = l.replace("\\B", " B")
    l = l.replace("\\K", " K")
    l = l.replace("\\M", " M")
    l = l.replace("\\T", " T")

    for k, v in kw.items():
        l = l.replace("\\%s" % k, v)

    if "\\" in l:
        print("WARN: unresolved char in", file=sys.stderr)
        print(" > %s" % l, file=sys.stderr)
        exit(1)

    abstract.append(l)

print("\n".join(abstract))


==> code/eval-sec-example.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{typedef} \PY{n+nf}{int} \PY{p}{(}\PY{o}{*}\PY{n}{FP\PYZus{}t}\PY{p}{)}\PY{p}{(}\PY{k+kt}{char} \PY{o}{*}\PY{p}{)}\PY{p}{;}
\PY{k+kt}{int} \PY{n+nf}{A}\PY{p}{(}\PY{k+kt}{char} \PY{o}{*}\PY{p}{)}\PY{p}{;}
\PY{k+kt}{int} \PY{n+nf}{B}\PY{p}{(}\PY{k+kt}{char} \PY{o}{*}\PY{p}{)}\PY{p}{;}

\PY{k+kt}{void} \PY{n+nf}{handleReq}\PY{p}{(}\PY{k+kt}{char} \PY{o}{*}\PY{n}{input}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{n}{FP\PYZus{}t}\PY{o}{*} \PY{n}{p1} \PY{o}{=} \PY{n}{malloc}\PY{p}{(}\PY{k}{sizeof}\PY{p}{(}\PY{n}{FP}\PY{p}{)}\PY{p}{)}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{eval}\PY{p}{:}\PY{n}{p1}\PY{p}{\PYZcb{}}\PY{err}{@}
  \PY{n}{FP\PYZus{}t}\PY{o}{*} \PY{n}{p2} \PY{o}{=} \PY{n}{malloc}\PY{p}{(}\PY{k}{sizeof}\PY{p}{(}\PY{n}{FP}\PY{p}{)}\PY{p}{)}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{eval}\PY{p}{:}\PY{n}{p2}\PY{p}{\PYZcb{}}\PY{err}{@}
  \PY{k+kt}{char} \PY{n}{buf}\PY{p}{[}\PY{l+m+mi}{10}\PY{p}{]}\PY{p}{;}

  \PY{n}{p1} \PY{o}{=} \PY{o}{\PYZam{}}\PY{n}{A}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{eval}\PY{p}{:}\PY{n}{p1assign}\PY{p}{\PYZcb{}}\PY{err}{@}
  \PY{n}{p2} \PY{o}{=} \PY{o}{\PYZam{}}\PY{n}{B}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{eval}\PY{p}{:}\PY{n}{p2assign}\PY{p}{\PYZcb{}}\PY{err}{@}
  
  \PY{c+c1}{// stack buffer overflow}
  \PY{n}{strcpy}\PY{p}{(}\PY{n}{buf}\PY{p}{,} \PY{n}{input}\PY{p}{)}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{eval}\PY{p}{:}\PY{n}{vuln}\PY{p}{\PYZcb{}}\PY{err}{@}
 
  \PY{p}{(}\PY{o}{*}\PY{n}{p1}\PY{p}{)}\PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{Hello}\PY{l+s}{\PYZdq{}}\PY{p}{)}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{eval}\PY{p}{:}\PY{n}{p1deref}\PY{p}{\PYZcb{}}\PY{err}{@}
  \PY{p}{(}\PY{o}{*}\PY{n}{p2}\PY{p}{)}\PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{PACTight!}\PY{l+s}{\PYZdq{}}\PY{p}{)}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{eval}\PY{p}{:}\PY{n}{p2deref}\PY{p}{\PYZcb{}}\PY{err}{@}
  
  \PY{n}{free}\PY{p}{(}\PY{n}{p1}\PY{p}{)}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{eval}\PY{p}{:}\PY{n}{p1free}\PY{p}{\PYZcb{}}\PY{err}{@}
  \PY{n}{free}\PY{p}{(}\PY{n}{p2}\PY{p}{)}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{eval}\PY{p}{:}\PY{n}{p2free}\PY{p}{\PYZcb{}}\PY{err}{@}
  \PY{k}{return}\PY{p}{;}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> code/nginx.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+cm}{/** ==== nginx/http/ngx\PYZus{}http\PYZus{}variables.h ==== */}
\PY{k}{typedef} \PY{k}{struct} \PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}s} \PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}t}\PY{p}{;}

\PY{c+c1}{// a function pointer type (i.e., sensitive type)}
\PY{k}{typedef} \PY{n+nf}{ngx\PYZus{}int\PYZus{}t} \PY{p}{(}\PY{o}{*}\PY{n}{ngx\PYZus{}http\PYZus{}get\PYZus{}variable\PYZus{}pt}\PY{p}{)}\PY{p}{(}\PY{p}{.}\PY{p}{.}\PY{p}{.}\PY{p}{)}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{fp2}\PY{p}{\PYZcb{}}\PY{err}{@}

\PY{k}{struct} \PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}s} \PY{p}{\PYZob{}} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{st}\PY{p}{\PYZcb{}}\PY{err}{@}
    \PY{n}{ngx\PYZus{}str\PYZus{}t}                 \PY{n}{name}\PY{p}{;}  
    \PY{c+c1}{// sensitive function pointer}
    \PY{n}{ngx\PYZus{}http\PYZus{}get\PYZus{}variable\PYZus{}pt}  \PY{n}{get\PYZus{}handler}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{stfp2}\PY{p}{\PYZcb{}}\PY{err}{@}
    \PY{c+c1}{// ...}
\PY{p}{\PYZcb{}}\PY{p}{;} \PY{c+c1}{// a sensitive data type}

\PY{c+cm}{/** ==== nginx/http/ngx\PYZus{}http\PYZus{}variables.c ==== */}
\PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}value\PYZus{}t} \PY{o}{*}
\PY{n+nf}{ngx\PYZus{}http\PYZus{}get\PYZus{}indexed\PYZus{}variable}\PY{p}{(}\PY{n}{ngx\PYZus{}http\PYZus{}request\PYZus{}t} \PY{o}{*}\PY{n}{r}\PY{p}{,} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{func}\PY{p}{\PYZcb{}}\PY{err}{@}
        \PY{n}{ngx\PYZus{}uint\PYZus{}t} \PY{n}{index}\PY{p}{)} \PY{p}{\PYZob{}}
    \PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}t}  \PY{o}{*}\PY{n}{v}\PY{p}{;} \PY{c+c1}{// sensitive pointer  @\PYZbs{}label\PYZob{}c:nginx:alloc\PYZcb{}@ }
    \PY{c+c1}{// ...}
    \PY{n}{v} \PY{o}{=} \PY{n}{cmcf}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{variables}\PY{p}{.}\PY{n}{elts}\PY{p}{;} \PY{c+c1}{// assignment of v @\PYZbs{}label\PYZob{}c:nginx:def\PYZcb{}@}
    \PY{c+c1}{// use of a sensitive point v}
    \PY{k}{if} \PY{p}{(}\PY{n}{v}\PY{p}{[}\PY{n}{index}\PY{p}{]}\PY{p}{.}\PY{n}{get\PYZus{}handler}\PY{p}{(}\PY{p}{.}\PY{p}{.}\PY{p}{.}\PY{p}{)} \PY{o}{=}\PY{o}{=} \PY{n}{NGX\PYZus{}OK}\PY{p}{)} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{use}\PY{p}{\PYZcb{}}\PY{err}{@}
    \PY{p}{\PYZob{}}
        \PY{c+c1}{// ...}
    \PY{p}{\PYZcb{}}
    \PY{c+c1}{// ...}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/povray.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{static} \PY{k+kt}{int} \PY{n+nf}{All\PYZus{}CSG\PYZus{}Intersect\PYZus{}Intersections} \PY{p}{(}\PY{n}{OBJECT} 
        \PY{o}{*}\PY{n}{Object}\PY{p}{,} \PY{n}{RAY} \PY{o}{*}\PY{n}{Ray}\PY{p}{,} \PY{n}{ISTACK} 
        \PY{o}{*}\PY{n}{Depth\PYZus{}Stack}\PY{p}{)}
\PY{p}{\PYZob{}}
  \PY{k+kt}{int} \PY{n}{Maybe\PYZus{}Found}\PY{p}{,} \PY{n}{Found}\PY{p}{;}
  \PY{n}{OBJECT} \PY{o}{*}\PY{n}{Current\PYZus{}Sib}\PY{p}{,} \PY{o}{*}\PY{n}{Inside\PYZus{}Sib}\PY{p}{;} \PY{c+c1}{//SENSITIVE @\PYZbs{}label\PYZob{}c:povray:sens\PYZcb{}@}
  \PY{n}{ISTACK} \PY{o}{*}\PY{n}{Local\PYZus{}Stack}\PY{p}{;}
  \PY{n}{INTERSECTION} \PY{o}{*}\PY{n}{Sibling\PYZus{}Intersection}\PY{p}{;}
  \PY{n}{Increase\PYZus{}Counter}\PY{p}{(}\PY{n}{stats}\PY{p}{[}\PY{n}{Ray\PYZus{}CSG\PYZus{}Intersection\PYZus{}}
          \PY{n}{Tests}\PY{p}{]}\PY{p}{)}\PY{p}{;}
  \PY{n}{Local\PYZus{}Stack} \PY{o}{=} \PY{n}{open\PYZus{}istack} \PY{p}{(}\PY{p}{)}\PY{p}{;}
  \PY{n}{Found} \PY{o}{=} \PY{n+nb}{false}\PY{p}{;}
  
  \PY{k}{for} \PY{p}{(}\PY{n}{Current\PYZus{}Sib} \PY{o}{=} \PY{p}{(}\PY{p}{(}\PY{n}{CSG} \PY{o}{*}\PY{p}{)}\PY{n}{Object}\PY{p}{)}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{Children}\PY{p}{;}  \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{povray}\PY{p}{:}\PY{n}{forloop1}\PY{p}{\PYZcb{}}\PY{err}{@}
          \PY{n}{Current\PYZus{}Sib} \PY{o}{!}\PY{o}{=} \PY{n+nb}{NULL}\PY{p}{;} \PY{n}{Current\PYZus{}Sib} 
          \PY{o}{=} \PY{n}{Current\PYZus{}Sib}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{Sibling}\PY{p}{)}
  \PY{p}{\PYZob{}}
     \PY{k}{if} \PY{p}{(}\PY{n}{Ray\PYZus{}In\PYZus{}Bound} \PY{p}{(}\PY{n}{Ray}\PY{p}{,} \PY{n}{Current\PYZus{}Sib}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{Bound}\PY{p}{)}\PY{p}{)} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{povray}\PY{p}{:}\PY{n}{if1}\PY{p}{\PYZcb{}}\PY{err}{@}
     \PY{p}{\PYZob{}}
        \PY{k}{if} \PY{p}{(}\PY{n}{All\PYZus{}Intersections} \PY{p}{(}\PY{n}{Current\PYZus{}Sib}\PY{p}{,} \PY{n}{Ray}\PY{p}{,} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{povray}\PY{p}{:}\PY{n}{if2}\PY{p}{\PYZcb{}}\PY{err}{@}
                \PY{n}{Local\PYZus{}Stack}\PY{p}{)}\PY{p}{)} 
    \PY{p}{\PYZob{}}
       \PY{k}{while} \PY{p}{(}\PY{p}{(}\PY{n}{Sibling\PYZus{}Intersection} \PY{o}{=} 
           \PY{n}{pop\PYZus{}entry}\PY{p}{(}\PY{n}{Local\PYZus{}Stack}\PY{p}{)}\PY{p}{)} \PY{o}{!}\PY{o}{=} \PY{n+nb}{NULL}\PY{p}{)}
       \PY{p}{\PYZob{}}  
          \PY{n}{Maybe\PYZus{}Found} \PY{o}{=} \PY{n+nb}{true}\PY{p}{;}
          \PY{k}{for} \PY{p}{(}\PY{n}{Inside\PYZus{}Sib} \PY{o}{=} \PY{p}{(}\PY{p}{(}\PY{n}{CSG} \PY{o}{*}\PY{p}{)}\PY{n}{Object}\PY{p}{)}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{povray}\PY{p}{:}\PY{n}{forloop2}\PY{p}{\PYZcb{}}\PY{err}{@}
                  \PY{n}{Children}\PY{p}{;} \PY{n}{Inside\PYZus{}Sib} 
                  \PY{o}{!}\PY{o}{=} \PY{n+nb}{NULL}\PY{p}{;} \PY{n}{Inside\PYZus{}Sib} \PY{o}{=} 
                  \PY{n}{Inside\PYZus{}Sib}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{Sibling}\PY{p}{)} 
          \PY{p}{\PYZob{}}
             \PY{k}{if} \PY{p}{(}\PY{n}{Inside\PYZus{}Sib} \PY{o}{!}\PY{o}{=} \PY{n}{Current\PYZus{}Sib}\PY{p}{)} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{povray}\PY{p}{:}\PY{n}{if3}\PY{p}{\PYZcb{}}\PY{err}{@}
         \PY{p}{\PYZob{}}  
            \PY{k}{if} \PY{p}{(}\PY{o}{!}\PY{p}{(}\PY{n}{Inside\PYZus{}Sib}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{Type} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{povray}\PY{p}{:}\PY{n}{if4}\PY{p}{\PYZcb{}}\PY{err}{@}
                 \PY{o}{\PYZam{}} \PY{n}{LIGHT\PYZus{}SOURCE\PYZus{}OBJECT}\PY{p}{)} 
                 \PY{o}{|}\PY{o}{|} \PY{p}{(}\PY{p}{(}\PY{n}{LIGHT\PYZus{}SOURCE} \PY{o}{*}\PY{p}{)}
                     \PY{n}{Inside\PYZus{}Sib}\PY{p}{)}
                          \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{Children}\PY{p}{)} 
                \PY{p}{\PYZob{}} 
               \PY{k}{if} \PY{p}{(}\PY{o}{!}\PY{n}{Inside\PYZus{}Object} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{povray}\PY{p}{:}\PY{n}{if5}\PY{p}{\PYZcb{}}\PY{err}{@}
                 \PY{p}{(}\PY{n}{Sibling\PYZus{}Intersection}
                  \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{IPoint}\PY{p}{,} \PY{n}{Inside\PYZus{}Sib}\PY{p}{)}\PY{p}{)} 
               \PY{p}{\PYZob{}}
                      \PY{n}{Maybe\PYZus{}Found} \PY{o}{=} \PY{n+nb}{false}\PY{p}{;}
                      \PY{k}{break}\PY{p}{;}
                   \PY{p}{\PYZcb{}}
            \PY{p}{\PYZcb{}}
             \PY{p}{\PYZcb{}}
          \PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/recursive-array.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{typedef} \PY{k}{struct} \PY{p}{\PYZob{}}
    \PY{k+kt}{int} \PY{n}{dummy1}\PY{p}{;}
        \PY{k+kt}{int} \PY{p}{(}\PY{o}{*}\PY{n}{coolFunct}\PY{p}{)}\PY{p}{(}\PY{p}{)}\PY{p}{;} 
    \PY{k+kt}{char} \PY{n}{dummy2}\PY{p}{;}
\PY{p}{\PYZcb{}} \PY{n}{Foo}\PY{p}{;}

\PY{k+kt}{int} \PY{n+nf}{main}\PY{p}{(}\PY{p}{)}
\PY{p}{\PYZob{}}
    \PY{p}{.}\PY{p}{.}\PY{p}{.}

    \PY{n}{Foo}\PY{o}{*} \PY{n}{list}\PY{p}{[}\PY{l+m+mi}{3}\PY{p}{]}\PY{p}{;}
    \PY{p}{.}\PY{p}{.}\PY{p}{.}
    
    \PY{c+c1}{//authenticatePAC(\PYZam{}list[0]);}
    \PY{c+c1}{//authenticatePAC(\PYZam{}list[0]\PYZhy{}\PYZgt{}coolFunct);}
    \PY{n}{list}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{coolFunct}\PY{p}{(}\PY{p}{)}\PY{p}{;}
    \PY{c+c1}{//addPAC(\PYZam{}list[0]\PYZhy{}\PYZgt{}coolFunct);}
    \PY{c+c1}{//addPAC(\PYZam{}list[0]);}
    
    \PY{c+c1}{//authenticatePAC(\PYZam{}list[1]);}
    \PY{c+c1}{//authenticatePAC(\PYZam{}list[1]\PYZhy{}\PYZgt{}coolFunct);}
    \PY{n}{list}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{coolFunct}\PY{p}{(}\PY{p}{)}\PY{p}{;}
    \PY{c+c1}{//addPAC(\PYZam{}list[1]\PYZhy{}\PYZgt{}coolFunct);}
    \PY{c+c1}{//addPAC(\PYZam{}list[1]);}

    \PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/recursive-struct.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{typedef} \PY{k}{struct} \PY{p}{\PYZob{}}
    \PY{k+kt}{int} \PY{n}{dummy1}\PY{p}{;}
    \PY{k+kt}{int} \PY{p}{(}\PY{o}{*}\PY{n}{coolFunct}\PY{p}{)}\PY{p}{(}\PY{p}{)}\PY{p}{;} 
    \PY{k+kt}{char} \PY{n}{dummy2}\PY{p}{;}
\PY{p}{\PYZcb{}} \PY{n}{Foo}\PY{p}{;}

\PY{k}{typedef} \PY{k}{struct} \PY{p}{\PYZob{}}
    \PY{n}{Foo} \PY{o}{*}\PY{n}{foo}\PY{p}{;}
    \PY{k+kt}{int} \PY{n}{dummy1}\PY{p}{;}
    \PY{k+kt}{char} \PY{n}{dumm2}\PY{p}{;} 
\PY{p}{\PYZcb{}} \PY{n}{Bar}\PY{p}{;}

\PY{k+kt}{int} \PY{n+nf}{main}\PY{p}{(}\PY{p}{)}
\PY{p}{\PYZob{}}
    \PY{p}{.}\PY{p}{.}\PY{p}{.}
    
    \PY{c+c1}{//authenticatePAC(\PYZam{}bar);}
    \PY{c+c1}{//authenticatePAC(\PYZam{}bar\PYZhy{}\PYZgt{}foo);}
    \PY{c+c1}{//authenticatePAC(\PYZam{}bar\PYZhy{}\PYZgt{}foo\PYZhy{}\PYZgt{}coolFunct); }
    \PY{n}{bar}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{foo}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{coolFunct}\PY{p}{(}\PY{p}{)}\PY{p}{;}
    \PY{c+c1}{//addPAC(\PYZam{}bar\PYZhy{}\PYZgt{}foo\PYZhy{}\PYZgt{}coolFunct);}
    \PY{c+c1}{//addPAC(\PYZam{}bar\PYZhy{}\PYZgt{}foo);}
    \PY{c+c1}{//addPAC(\PYZam{}bar);}

    \PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/sensitive-nginx.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+cm}{/** == Example of sensitive pointer }
\PY{c+cm}{ * protection in NGINX== **/}

\PY{c+c1}{// nginx/http/ngx\PYZus{}http\PYZus{}variables.h}
\PY{k}{typedef} \PY{k}{struct} \PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}s}  
            \PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}t}\PY{p}{;}

\PY{k}{typedef} \PY{n+nf}{void} \PY{p}{(}\PY{o}{*}\PY{n}{ngx\PYZus{}http\PYZus{}set\PYZus{}variable\PYZus{}pt}\PY{p}{)} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{fp1}\PY{p}{\PYZcb{}}\PY{err}{@}
    \PY{p}{(}\PY{n}{ngx\PYZus{}http\PYZus{}request\PYZus{}t} \PY{o}{*}\PY{n}{r}\PY{p}{,} 
     \PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}value\PYZus{}t} \PY{o}{*}\PY{n}{v}\PY{p}{,} 
     \PY{k+kt}{uintptr\PYZus{}t} \PY{n}{data}\PY{p}{)}\PY{p}{;}  \PY{c+c1}{// Sensitive!}
\PY{k}{typedef} \PY{n+nf}{ngx\PYZus{}int\PYZus{}t} \PY{p}{(}\PY{o}{*}\PY{n}{ngx\PYZus{}http\PYZus{}get\PYZus{}variable\PYZus{}pt}\PY{p}{)} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{fp2}\PY{p}{\PYZcb{}}\PY{err}{@}
    \PY{p}{(}\PY{n}{ngx\PYZus{}http\PYZus{}request\PYZus{}t} \PY{o}{*}\PY{n}{r}\PY{p}{,}             
     \PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}value\PYZus{}t} \PY{o}{*}\PY{n}{v}\PY{p}{,} 
     \PY{k+kt}{uintptr\PYZus{}t} \PY{n}{data}\PY{p}{)}\PY{p}{;} \PY{c+c1}{// Sensitive!}
\PY{p}{.}\PY{p}{.}\PY{p}{.}

\PY{k}{struct} \PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}s} \PY{p}{\PYZob{}} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{st}\PY{p}{\PYZcb{}}\PY{err}{@}
    \PY{n}{ngx\PYZus{}str\PYZus{}t}                 \PY{n}{name}\PY{p}{;}  
    \PY{n}{ngx\PYZus{}http\PYZus{}set\PYZus{}variable\PYZus{}pt}  \PY{n}{set\PYZus{}handler}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{stfp1}\PY{p}{\PYZcb{}}\PY{err}{@}\PY{c+c1}{// Sensitive!}
    \PY{n}{ngx\PYZus{}http\PYZus{}get\PYZus{}variable\PYZus{}pt}  \PY{n}{get\PYZus{}handler}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{stfp2}\PY{p}{\PYZcb{}}\PY{err}{@}\PY{c+c1}{// Sensitive!}
    \PY{k+kt}{uintptr\PYZus{}t}                 \PY{n}{data}\PY{p}{;}
    \PY{n}{ngx\PYZus{}uint\PYZus{}t}                \PY{n}{flags}\PY{p}{;}
    \PY{n}{ngx\PYZus{}uint\PYZus{}t}                \PY{n}{index}\PY{p}{;}
\PY{p}{\PYZcb{}}\PY{p}{;} \PY{c+c1}{// Sensitive struct!}


\PY{c+c1}{// nginx/http/ngx\PYZus{}http\PYZus{}variables.c}
\PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}value\PYZus{}t} \PY{o}{*}
\PY{n+nf}{ngx\PYZus{}http\PYZus{}get\PYZus{}indexed\PYZus{}variable}\PY{p}{(}\PY{n}{ngx\PYZus{}http\PYZus{}request\PYZus{}t} \PY{o}{*}\PY{n}{r}\PY{p}{,} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{func}\PY{p}{\PYZcb{}}\PY{err}{@}
        \PY{n}{ngx\PYZus{}uint\PYZus{}t} \PY{n}{index}\PY{p}{)} 
\PY{p}{\PYZob{}}
    \PY{n}{ngx\PYZus{}http\PYZus{}variable\PYZus{}t}        \PY{o}{*}\PY{n}{v}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{alloc}\PY{p}{\PYZcb{}}\PY{err}{@}\PY{c+c1}{// Sensitive!}
    \PY{p}{.}\PY{p}{.}\PY{p}{.}

    \PY{n}{v} \PY{o}{=} \PY{n}{cmcf}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{variables}\PY{p}{.}\PY{n}{elts}\PY{p}{;} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{def}\PY{p}{\PYZcb{}}\PY{err}{@}\PY{c+c1}{// Assignment of v}
    \PY{p}{.}\PY{p}{.}\PY{p}{.}
    \PY{c+c1}{// Uses of v are protected}
    \PY{k}{if} \PY{p}{(}\PY{n}{v}\PY{p}{[}\PY{n}{index}\PY{p}{]}\PY{p}{.}\PY{n}{get\PYZus{}handler}\PY{p}{(}\PY{n}{r}\PY{p}{,} \PY{o}{\PYZam{}}\PY{n}{r}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{variables}\PY{p}{[}\PY{n}{index}\PY{p}{]}\PY{p}{,} \PY{err}{@}\PY{err}{\PYZbs{}}\PY{n}{label}\PY{p}{\PYZob{}}\PY{n+nl}{c}\PY{p}{:}\PY{n+nl}{nginx}\PY{p}{:}\PY{n}{use}\PY{p}{\PYZcb{}}\PY{err}{@}
            \PY{n}{v}\PY{p}{[}\PY{n}{index}\PY{p}{]}\PY{p}{.}\PY{n}{data}\PY{p}{)} \PY{o}{=}\PY{o}{=} \PY{n}{NGX\PYZus{}OK}\PY{p}{)}
    \PY{p}{\PYZob{}}
        \PY{k}{if} \PY{p}{(}\PY{n}{v}\PY{p}{[}\PY{n}{index}\PY{p}{]}\PY{p}{.}\PY{n}{flags} \PY{o}{\PYZam{}} \PY{n}{NGX\PYZus{}HTTP\PYZus{}VAR\PYZus{}NOCACHEABLE}\PY{p}{)} \PY{p}{\PYZob{}}
        \PY{n}{r}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{variables}\PY{p}{[}\PY{n}{index}\PY{p}{]}\PY{p}{.}\PY{n}{no\PYZus{}cacheable} \PY{o}{=} \PY{l+m+mi}{1}\PY{p}{;}
    \PY{p}{\PYZcb{}}
    \PY{k}{return} \PY{o}{\PYZam{}}\PY{n}{r}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{variables}\PY{p}{[}\PY{n}{index}\PY{p}{]}\PY{p}{;}
    \PY{p}{\PYZcb{}}
    \PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/sensitive.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+cm}{/** == Example of which sensitive pointers are protected == **/}
\PY{k}{typedef} \PY{k}{struct} \PY{p}{\PYZob{}}
    \PY{k+kt}{int} \PY{n}{dummy1}\PY{p}{;}
    \PY{k}{volatile} \PY{n+nf}{int} \PY{p}{(}\PY{o}{*}\PY{n}{coolFunct}\PY{p}{)}\PY{p}{(}\PY{p}{)}\PY{p}{;} \PY{c+c1}{// Code pointer (sensitive!)}
    \PY{k+kt}{char} \PY{n}{dummy2}\PY{p}{;}
\PY{p}{\PYZcb{}} \PY{n}{Foo}\PY{p}{;} \PY{c+c1}{// Sensitive!}

\PY{k}{typedef} \PY{k}{struct} \PY{p}{\PYZob{}}
    \PY{k}{volatile} \PY{n}{Foo}\PY{o}{*} \PY{n}{foo}\PY{p}{;} \PY{c+c1}{// Sensitive!}
    \PY{k+kt}{int} \PY{n}{dummy1}\PY{p}{;}
    \PY{k+kt}{char} \PY{n}{dummy2}\PY{p}{;}
\PY{p}{\PYZcb{}} \PY{n}{Bar}\PY{p}{;} \PY{c+c1}{// Sensitive! }

\PY{k}{typedef} \PY{k}{struct} \PY{p}{\PYZob{}}
    \PY{k+kt}{int} \PY{n}{x}\PY{p}{;}
    \PY{k+kt}{int} \PY{n}{d}\PY{p}{;}
    \PY{k+kt}{char} \PY{n}{c}\PY{p}{;}
\PY{p}{\PYZcb{}} \PY{n}{Bez}\PY{p}{;} \PY{c+c1}{// Not Sensitive!}
\end{Verbatim}


==> data/nbench.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\scriptsize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,2304.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(516,934){\makebox(0,0)[r]{\strut{}$-1$}}%
      \csname LTb\endcsname%%
      \put(516,1142){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \csname LTb\endcsname%%
      \put(516,1350){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(516,1559){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \csname LTb\endcsname%%
      \put(516,1767){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(516,1975){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \csname LTb\endcsname%%
      \put(516,2183){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(948,862){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Numeric Sort}}}%
      \csname LTb\endcsname%%
      \put(1308,862){\rotatebox{45}{\makebox(0,0)[r]{\strut{}String Sort}}}%
      \csname LTb\endcsname%%
      \put(1667,862){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Bitfield}}}%
      \csname LTb\endcsname%%
      \put(2027,862){\rotatebox{45}{\makebox(0,0)[r]{\strut{}FP emulation}}}%
      \csname LTb\endcsname%%
      \put(2387,862){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Fourier}}}%
      \csname LTb\endcsname%%
      \put(2747,862){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Assignment}}}%
      \csname LTb\endcsname%%
      \put(3107,862){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Idea}}}%
      \csname LTb\endcsname%%
      \put(3467,862){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Huffman}}}%
      \csname LTb\endcsname%%
      \put(3826,862){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Neural}}}%
      \csname LTb\endcsname%%
      \put(4186,862){\rotatebox{45}{\makebox(0,0)[r]{\strut{}LU Decomposition}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(114,1558){\rotatebox{-270}{\makebox(0,0){\strut{}Performance Overhead (\%)}}}%
      \csname LTb\endcsname%%
      \put(4015,2046){\makebox(0,0)[r]{\strut{}PACTight-return}}%
      \csname LTb\endcsname%%
      \put(4015,1898){\makebox(0,0)[r]{\strut{}PACTight-CFI+VTable}}%
      \csname LTb\endcsname%%
      \put(4015,1750){\makebox(0,0)[r]{\strut{}PACTight-CPI(inc. CFI+VTable+return)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/nbench}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> data/opt-impact.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\scriptsize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5182.00,2304.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(444,907){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(444,1057){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%%
      \put(444,1206){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%%
      \put(444,1356){\makebox(0,0)[r]{\strut{}$60$}}%
      \csname LTb\endcsname%%
      \put(444,1506){\makebox(0,0)[r]{\strut{}$80$}}%
      \csname LTb\endcsname%%
      \put(444,1655){\makebox(0,0)[r]{\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(444,1805){\makebox(0,0)[r]{\strut{}$120$}}%
      \csname LTb\endcsname%%
      \put(728,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}400.perlbench}}}%
      \csname LTb\endcsname%%
      \put(940,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}401.bzip2}}}%
      \csname LTb\endcsname%%
      \put(1152,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}403.gcc}}}%
      \csname LTb\endcsname%%
      \put(1363,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}429.mcf}}}%
      \csname LTb\endcsname%%
      \put(1575,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}433.milc}}}%
      \csname LTb\endcsname%%
      \put(1787,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}444.namd}}}%
      \csname LTb\endcsname%%
      \put(1999,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}445.gobmk}}}%
      \csname LTb\endcsname%%
      \put(2211,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}447.dealII}}}%
      \csname LTb\endcsname%%
      \put(2423,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}450.soplex}}}%
      \csname LTb\endcsname%%
      \put(2635,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}453.povray}}}%
      \csname LTb\endcsname%%
      \put(2846,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}456.hmmer}}}%
      \csname LTb\endcsname%%
      \put(3058,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}462.libquantum}}}%
      \csname LTb\endcsname%%
      \put(3270,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}458.sjeng}}}%
      \csname LTb\endcsname%%
      \put(3482,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}464.h264ref}}}%
      \csname LTb\endcsname%%
      \put(3694,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}470.lbm}}}%
      \csname LTb\endcsname%%
      \put(3906,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}471.omnetpp}}}%
      \csname LTb\endcsname%%
      \put(4118,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}473.astar}}}%
      \csname LTb\endcsname%%
      \put(4329,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}482.sphinx3}}}%
      \csname LTb\endcsname%%
      \put(4541,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}483.xalancbmk}}}%
      \csname LTb\endcsname%%
      \put(4753,760){\rotatebox{45}{\makebox(0,0)[r]{\strut{}Average-SPEC}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(114,1318){\rotatebox{-270}{\makebox(0,0){\strut{}Performance overhead (\%)}}}%
      \csname LTb\endcsname%%
      \put(2173,2146){\makebox(0,0)[r]{\strut{}LTO/INLN/OVWRT}}%
      \csname LTb\endcsname%%
      \put(2173,1957){\makebox(0,0)[r]{\strut{}LTO/INLN}}%
      \csname LTb\endcsname%%
      \put(3916,2146){\makebox(0,0)[r]{\strut{}LTO/No INLN}}%
      \csname LTb\endcsname%%
      \put(3916,1957){\makebox(0,0)[r]{\strut{}No LTO/No INLN}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/opt-impact}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> eval-anal.tex <==
\subsection{Performance Analysis}
\label{s:eval:anal}

\TODO{Add justification for high overhead benchmarks}


==> eval-sec-prop.tex <==
% ### Security analysis
% - Vulnerable code example and showcase all three properties on it.
% - control flow hijack is critical. Control flow hijack description and how it happens due to a memory corruption error.
\subsubsection{Achieving the Security Properties}
\sys's security foundation is in the three properties previously discussed in
~\autoref{s:design:prop}. Thus, we take a closer look at a code example, explain
possible vulnerabilities to each of the three properties, and demonstrate
that \sys enforces each of the properties.

~\autoref{c:sec-eval} shows a vulnerable code snippet that can be violated in a
variety of ways. The attacker's main goal in exploiting this code is to divert 
(\cc{p1}) and (\cc{p2}) from their proper control-flow. We assume the attacker has 
the same capabilities discussed in ~\autoref{s:threat}. The attacker will utilize
the memory corruption vulnerability in Line~\ref{c:eval:vuln}. We showcase three 
scenarios for each of the three properties in which the attacker can violate 
the control-flow, and how \sys defends against each.

\begin{itemize}[leftmargin=*]
%
\item Scenario 1: In this scenario, the attacker can attempt to directly 
overwrite (\cc{p1}) or (\cc{p2}) with another address that points to an arbitrary
location in memory. This location may be a gadget chain that executes the attack
logic when the pointers get dereferenced in Lines~\ref{c:eval:p1deref} and 
\ref{c:eval:p2deref}. This attack violates the (\emph{unforgeability}) property. 
\sys defends against this due to the PAC mechanism. Before the pointers get
dereferenced, \pctauth will detect the violation.
%
\item Scenario 2: The attacker can't simply overwrite. Thus, in this scenario, 
the attacker can attempt to overwrite (\cc{p2}) with (\cc{p1}) and redirect \cc{p2}'s 
dereference to execute function (\cc{A}) instead of function (\cc{B}). This attack 
can occur even with a PACed pointer \cite{parts-lilijestrand-sec19}. This attack 
violates the (\emph{non-copyability}) property. However, \sys defends against this 
due to the use of the location (\cc{\&p}) in the modifier. This means that 
\pctauth will generate a different modifier from the one already there and the 
violation will be detected.
%
\item Scenario 3: The attacker can't overwrite nor copy any legitimate pointers.
In this last resort scenario, the attacker can attempt to reuse the pointers after
they have been freed in Lines~\ref{c:eval:p1free} and \ref{c:eval:p2free}.
This attack violates the (\emph{non-dangling}) property. \sys defends against this, since
\pctrmtag removes the metadata before \cc{free}. Thus, when the attacker attempts to
reuse the freed pointer, \pctauth will detect that no metadata is present for that 
pointer and generate an exception.
\end{itemize}

\begin{figure}[t!]
        \inputminted[xleftmargin=11pt,fontsize=\scriptsize,linenos,escapeinside=@@]{cpp}{code/eval-sec-example.c}
        \caption{Vulnerable code example}
        \label{c:sec-eval}
\end{figure}




==> figs/tbl-eor.tex <==
\begin{tabular}{llllclll}
	\cline{4-5}
	 &  &  & \textbf{Instructions} & \multicolumn{1}{l}{\textbf{Mac Mini M1 time (ns)}} &  &  &  \\ \cline{4-5}
	  &  &  & \cc{pacia}                 & 2.1963                                             &  &  &  \\ \cline{4-5}
	   &  &  & \cc{autia}                 & 2.1890                                             &  &  &  \\ \cline{4-5}
	    &  &  & Six \cc{EOR}               & 1.9782                                             &  &  &  \\ \cline{4-5}
	     &  &  & Seven \cc{EOR}             & 2.1894                                             &  &  &  \\ \cline{4-5}
	      &  &  & Eight \cc{EOR}             & 2.5016                                             &  &  &  \\ \cline{4-5}
\end{tabular}


==> figs/tbl-geo.tex <==
\begin{tabular}{llcll}
\hline
\multicolumn{1}{c}{\textbf{Mechanism}} & \textbf{SPEC2006} & \multicolumn{1}{l}{\textbf{nbench}} & \textbf{CoreMark} & \textbf{All} \\ \hline
\sys-Return & 0.64 & 0.07 & 0.2  & \textbf{0.43} \\ \hline
\sys-CFI+VTable+Return    & 1.57 & 0.12 & 0.34 & \textbf{1.03} \\ \hline
\sys-CPI    & 6.97 & 0.21 & 0.66 & \textbf{4.41} \\ \hline
\end{tabular}



==> figs/tbl-loc.tex <==
\begin{tabular}{lrrr}
\toprule
  % first line
  \multirow{2}{*}{\textbf{Module}} &
  \multicolumn{3}{c}{\textbf{Lines of Code}}
  \\
  \cmidrule(r){2-4}
  % second line
  &
  \textbf{Added} &
  \textbf{Deleted} &
  \textbf{Total}
  \\
\midrule
  \sys Library    &  656 &  0 &  656 \\
  LLVM Pass   &  3216 & 21 &  3237 \\
  AArch64 Backend           & 109 & 12 & 121 \\
\midrule
  \textbf{Total} & 3981 & 33 & 4014 \\
\bottomrule
\end{tabular}


==> figs/tbl-nginx.tex <==
\begin{tabular}{llllll}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}No. of \\ workers\end{tabular}}} &
  \textbf{Baseline} &
  \multicolumn{2}{l}{\textbf{\sys-CFI}} &
  \multicolumn{2}{l}{\textbf{\sys-CPI}} \\ \cline{2-6} 
 &
  Req\textbackslash{}sec &
  Req\textbackslash{}sec &
  Overhead &
  Req\textbackslash{}sec &
  Overhead \\ \hline
4 &
  95.9 &
  \multicolumn{1}{c}{92.01} &
  4\% &
  \multicolumn{1}{c}{90.84} &
  5.57\% \\ \hline
\end{tabular}


==> figs/tbl-pac-instr.tex <==
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{} &
  \multicolumn{1}{c|}{\textbf{Type}} &
  \multicolumn{1}{c|}{\textbf{Instruction}} &
  \multicolumn{1}{c|}{\textbf{Key used}} \\ \hline
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Signing\\ Instructions\end{tabular}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Code\\ Pointers\end{tabular}}} &
	  \cc{PACIA} &
  A \\ \cline{3-4} 
 &
 &
	\cc{PACIB} &
  B \\ \cline{2-4} 
 &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Data\\ Pointers\end{tabular}}} &
	  \cc{PACDA} &
  A \\ \cline{3-4} 
 &
 &
	\cc{PACDB} &
  B \\ \cline{2-4} 
 &
 \textbf{Generic} &
	\cc{PACGA} &
  A \\ \hline
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Authenticating\\ Instructions\end{tabular}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Code\\ Pointers\end{tabular}}} &
	  \cc{AUTIA} &
  A \\ \cline{3-4} 
 &
 &
	\cc{AUTIB} &
  B \\ \cline{2-4} 
 &
  \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Data\\ Pointers\end{tabular}}}} &
	  \cc{AUTDA} &
  A \\ \cline{3-4} 
 &
  \multicolumn{1}{l|}{} &
	\cc{AUTDB} &
 B \\ \hline
 \textbf{\begin{tabular}[c]{@{}l@{}}Stripping \\ Instruction\end{tabular}} &
  \multicolumn{1}{l|}{\textbf{All types}} &
	\cc{XPAC**} &
 - \\ \hline
\end{tabular}







\if 0
\begin{tabular}{|l|l|l|l|}
	\hline
	\textbf{Instruction} & \textbf{Key used} & \textbf{Pointer type} & \textbf{Purpose}  	\\ \hline
	\cc{PACIA}                & A.Code            & Code                  & Sign              	\\ \hline
	\cc{PACIB}                & B.Code            & Code                  & Sign             	\\ \hline
	\cc{PACDA}                & A.Data            & Data                  & Sign             	\\ \hline
	\cc{PACDB}                & B.Data            & Data                  & Sign             	\\ \hline
	\cc{AUTIA}                & A.Code            & Code                  & Authenticate     	\\ \hline
	\cc{AUTIB}                & B.Code            & Code                  & Authenticate       \\ \hline
	\cc{AUTDA}                & A.Data            & Data                  & Authenticate       \\ \hline
	\cc{AUTDB}                & B.Data            & Data                  & Authenticate       \\ \hline
	\cc{PACGA}               & Generic           & Generic               & Generic            \\ \hline
	\cc{XPAC**}               &                   &                       & PAC Stripping      \\ \hline
\end{tabular}
\fi


==> figs/tbl-pactight-keys.tex <==
\begin{tabular}{|l|c|c|}
	\hline
	\textbf{} &
	  \multicolumn{1}{l|}{\textbf{Key used}} &
	    \multicolumn{1}{l|}{\textbf{Instructions used}} \\ \hline
		Sensitive data pointer & Data A & PACDA/AUTDA \\ \hline
		\begin{tabular}[c]{@{}l@{}}Sensitive code pointer \\ (Function pointer)\end{tabular} & Code A & PACIA/AUTIA \\ \hline
		\begin{tabular}[c]{@{}l@{}}Sensitive code pointer \\ (Return address)\end{tabular} & Code B & PACIB/AUTIB \\ \hline
\end{tabular}


==> figs/tbl-properties.tex <==
\begin{tabular}{|l|c|c|c|}
	\hline
	\textbf{Defense} & \multicolumn{1}{l|}{\textbf{Property 1}} & \multicolumn{1}{l|}{\textbf{Property 2}} & \multicolumn{1}{l|}{\textbf{Property 3}} \\ \hline
	GCC              & \textbf{X}                               & \textbf{}                                & \textbf{}                                \\ \hline
	Apple Clang      & \textbf{X}                               & \textbf{}                                & \textbf{}                                \\ \hline
	PARTS            & \textbf{X}                               & \textbf{}                                & \textbf{}                                \\ \hline
	PACStack         & \textbf{X}                               & \textbf{X}                               & \textbf{}                                \\ \hline
	PCan             & \textbf{X}                               & \textbf{}                                & \textbf{}                                \\ \hline
	PTAuth           & \textbf{X}                               & \textbf{}                                & \textbf{X}                               \\ \hline
	\sys             & \textbf{X}                               & \textbf{X}                               & \textbf{X}                               \\ \hline
\end{tabular}


==> figs/tbl-relwk-v.tex <==
\CH{
		\begin{tabular}{l|lll|l}
			\textbf{Defense}                                                                           & PARTS-CFI & PACStack & PTAuth & \textbf{PACTight} \\ \hline
			\textbf{\begin{tabular}[c]{@{}l@{}}Protection \\ scope\end{tabular}} &
				  \begin{tabular}[c]{@{}l@{}}Return addresses\\ and indirect code\\ pointers\end{tabular} &
					    \begin{tabular}[c]{@{}l@{}}Return \\ addresses\end{tabular} &
						      \begin{tabular}[c]{@{}l@{}}Heap \\ allocated\\ objects\end{tabular} &
							        \begin{tabular}[c]{@{}l@{}}Return addresses\\ and sensitive\\ pointers\end{tabular} \\ \cline{1-1}
									\textbf{\begin{tabular}[c]{@{}l@{}}Attacker\\ abilities\end{tabular}} &
										  \begin{tabular}[c]{@{}l@{}}Arbitrary\\ read-write\end{tabular} &
											    \begin{tabular}[c]{@{}l@{}}Arbitrary\\ read-write\end{tabular} &
												      \begin{tabular}[c]{@{}l@{}}Arbitrary\\ write\end{tabular} &
													        \begin{tabular}[c]{@{}l@{}}Arbitrary\\ read-write\end{tabular} \\ \cline{1-1}
															\textbf{\begin{tabular}[c]{@{}l@{}}PAC \\ modifier\end{tabular}} &
																  \begin{tabular}[c]{@{}l@{}}SP for return \\ addresses \\ and type-id \\ for indirect \\ code pointers.\end{tabular} &
																	    \begin{tabular}[c]{@{}l@{}}Previous \\ return \\ address \\ on the \\ stack\end{tabular} &
																		      \begin{tabular}[c]{@{}l@{}}A \\ generated \\ object-id\end{tabular} &
																			        \begin{tabular}[c]{@{}l@{}}Previous return \\ address and a \\ unique function \\ id for return \\ addresses. The \\ location of the \\ pointer and a \\ random tag for \\ sensitive pointers.\end{tabular} \\ \cline{1-1}
																					\textbf{\begin{tabular}[c]{@{}l@{}}Pointer \\ cannot\\ be forged\end{tabular}}             & Yes       & Yes      & Yes    & Yes               \\ \cline{1-1}
																						\textbf{\begin{tabular}[c]{@{}l@{}}Pointer \\ cannot\\ be replayed\end{tabular}}           & No        & Yes      & No     & Yes               \\ \cline{1-1}
																							\textbf{\begin{tabular}[c]{@{}l@{}}Dangling \\ pointer\\ cannot \\ be reused\end{tabular}} & No        & No       & Yes    & Yes               \\ \hline
		\end{tabular}
}


==> opt.tex <==
\section{\sys Optimizations}
\label{s:opt}



